Optimal subsampling designs

Subsampling is commonly used to overcome computational and economical bottlenecks in the analysis of finite populations and massive datasets. Existing methods are often limited in scope and use optimality criteria (e.g., A-optimality) with well-known deficiencies, such as lack of invariance to the measurement-scale of the data and parameterisation of the model. A unified theory of optimal subsampling design is still lacking. We present a theory of optimal design for general data subsampling problems, including finite population inference, parametric density estimation, and regression modelling. Our theory encompasses and generalises most existing methods in the field of optimal subdata selection based on unequal probability sampling and inverse probability weighting. We derive optimality conditions for a general class of optimality criteria, and present corresponding algorithms for finding optimal sampling schemes under Poisson and multinomial sampling designs. We present a novel class of transformation- and parameterisation-invariant linear optimality criteria which enjoy the best of two worlds: the computational tractability of A-optimality and invariance properties similar to D-optimality. The methodology is illustrated on an application in the traffic safety domain. In our experiments, the proposed invariant linear optimality criteria achieve 92-99% D-efficiency with 90-95% lower computational demand. In contrast, the A-optimality criterion has only 46% and 60% D-efficiency on two of the examples.

==> old.tex <==
%In contrast to D- and $d_{\mathrm{S}}$-optimality, the $d_{\mathrm{ER}}$-optimality criterion is for this problem not invariant under affine transformations of the data. The reason is that the defining equation \eqref{eq:theta0_fps} is under-specified, in the sense that it does not contain any second moment information (i.e., no covariance parameters). 


%Of course, this is not possible in practice. A rigorous treatment of this issue may be found in \citet{Imberg2022b}.


%An implementation of a sequential optimal subsampling method with respect to the c-optimality criterion has also been presented for this application in \citet{Imberg2022b}.


%Some concluding remarks are provided in Section \ref{sec:remarks}.


%Indeed, $\tilde{c}_i$ can in this case be evaluated solely as a function of $\{\boldsymbol{x}_i\}_{i \in \mathcal D}$. 


%We resist to present a more detailed description of sequential optimal design algorithms, since many variations exist and the most appropriate implementation vary depending on context. 
%All steps in Algorithm \ref{alg:sequential_optimal_designs} may not be needed or implemented in the same order in all applications. 
%$^{\dagger}$Use uniform sampling scheme if sufficient information to evaluate the anticipated covariance matrix is not yet available (e.g., if $k = 1$). 


%In our last step towards practically implementable optimal subsampling designs, we describe how the information needed to derive an optimal sampling scheme may be acquired gradually during the sampling process using multi-stage sampling procedures and sequential optimal design.


%It is a hypothetical construct we use to define an objective function for an optimisation problem that depends on fixed characteristics of the data that we cannot afford to observe. 


%We do, however, assume that some information about the members $i \in \mathcal D$ is available at the design stage. Finding an optimal design would not be possible otherwise. 


%, which implies that the L-matrices in Proposition \ref{prop:MD_ER_KL} may be takes as $k\mathbf{I}_{p \times p}$ for some $k \ne 0$.


%It is particularly suitable as optimality criterion for subsampling problems as it measures the performance of the estimator $\hat{\boldsymbol{\theta}}_{\!\boldsymbol{\mu}}$ by the same metric as the one used to define the target characteristic $\boldsymbol{\theta}_0$.  
%The  \textit{d}-optimality criterion has, however, a broader is applicable more generally.  and arguably more appropriate for more g
%also beyond regmore generally, and also more appropriate for non-linear or non-homoscedastic models as the it measures the performance of the estimator $\hat{\boldsymbol{\theta}}_{\!\boldsymbol{\mu}}$ by the same metric used to define the target characteristic $\boldsymbol{\theta}_0$.  
%Beyond ordinary least squares, the \textit{d}-optimality criterion with the empirical risk distance is often more appropriate, as it measures the performance of the estimator $\hat{\boldsymbol{\theta}}_{\!\boldsymbol{\mu}}$ by the same metric as the one used to define the target characteristic $\boldsymbol{\theta}_0$.  

%By the result of Proposition \ref{prop:equivalence}, any differentiable $\Phi$-optimality criterion may be represented as a \textit{d}-optimality criterion, and vice versa. The reason for introducing \textit{d}-optimality is therefore not to enlarge the class of optimality criteria under consideration but rather to present an alternative perspective on optimal design. 


%, which are simultaneously fulfilled for the $\Phi$-optimality criterion and corresponding \textit{d}-optimality criterion. Proposition \ref{prop:equivalence}\ref{prop:equivalence_a} follows immediately by definition of d- and L-optimality.

 
 %We wish to obtain an accurate estimate of the full-data parameter $\boldsymbol{\theta}_0$, i.e., the parameter estimate that we would have been obtained if inference based on the full data $(\boldsymbol{x}_i, \boldsymbol{y}_i)_{i\in \mathcal D}$ had been feasible.
 % \footnotesize
    % $^{\dagger}$Optimality conditions \eqref{eq:mui} or \eqref{eq:powor_a}–\eqref{eq:powor_c} fulfilled ($|\frac{1}{2}\log (c_i/c_j) - \log (\mu_{t,i}/\mu_{t,j})| < \Delta$ for all $i,j, \in \mathcal D\setminus \mathcal E$ and $|\frac{1}{2}\log (c_i/c_j) + \log \mu_{t,j}| > \Delta$ for all $i \in \mathcal E, j \in \mathcal D \setminus \mathcal E$, where $\mathcal E = \{i \in \mathcal D: \mu_{t,i} = 1\}$ for PO-WOR and $\mathcal E = \varnothing$ otherwise) or relative improvement of objective function less than $\epsilon$.
    
    % \IF{PO-WOR and $\{i \in \mathcal D: \mu_{t,i} = 1\} \ne \varnothing$}
        %     \STATE Let $\mathcal E = \{i \in \mathcal D: \mu_{t,i} = 1\}$.
        %     \STATE Let $\delta_{1,t} = \max_{i \in \mathcal D \setminus \mathcal E} \{\frac{1}{2}\log c_i - \log \mu_{t,i}\} - \min_{j \in \mathcal D \setminus \mathcal E} \{\frac{1}{2}\log c_j - \log\mu_{t,j}\}$.
        %     \STATE Let $\delta_{2,t}  = \max_{i \in \mathcal D \setminus \mathcal E} \{\frac{1}{2}\log c_i - \log \mu_{t,i}\} - \min_{j \in \mathcal E} \{\frac{1}{2}\log c_j\}$.
        % \ELSE 
        %     \STATE Let $\delta_{1,t} = \max_{i \in \mathcal D} \{\frac{1}{2}\log c_i - \log \mu_{t,i}\} - \min_{j \in \mathcal D} \{\frac{1}{2}\log c_j - \log\mu_{t,j}\}$.
        %     \STATE Let $\delta_{2,t} = 0$.
        % \ENDIF         
        % \STATE \textbf{If} $\max\{\delta_{1,t}, \delta_{2,t}\} < \Delta$ \textbf{then} Go to \footnotesize{\ref{step:end}}.
        % \STATE \textbf{Else if} $t>1$ and  $|\Phi(\boldsymbol{\Gamma}(\boldsymbol{\mu}_t; \boldsymbol{\theta}_0)) - \Phi(\boldsymbol{\Gamma}(\boldsymbol{\mu}_{t-1}; \boldsymbol{\theta}_0))|/ |\Phi(\boldsymbol{\Gamma}(\boldsymbol{\mu}_{t-1}; \boldsymbol{\theta}_0))| < \varepsilon$
        % \textbf{then } Go to \footnotesize{\ref{step:end}}.
        % \STATE \textbf{Else if} $t>1$ and ($\delta_{1,t}> \delta_{1,t-1}$ or $\delta_{2,t} > \delta_{2,t-1}$)
        % \textbf{then } Go to \footnotesize{\ref{step:end}}.
        
        %Optimal sampling scheme $\boldsymbol{\mu}^*$ with $\mu_i^*> 0$ for all $i \in \mathcal D$ does not exist. 

    % \IF{Algorithm converged} 
    %     \STATE \textbf{Return} $\boldsymbol{\mu}_t$.
    % \ENDIF
    % \medskip \\
    % \textbf{Output:} 
    % \medskip \\  
    % \IF{any $c_i$ = 0}
    %     \label{step:end}
    %     \STATE Algorithm did not converge, $c_i = 0$ encountered. 
    % \ELSIF{$t < T$ and ($\delta_{1,t}> \delta_{1,t-1}$ or $\delta_{2,t} > \delta_{2,t-1}$)}
    %     \STATE Algorithm diverged. 
    % \ELSIF{$t = T$ and $\max\{\delta_{1,t}, \delta_{2,t}\} > \Delta$}
    %     \STATE Algorithm did not converge. Maximal number of iterations reached. 
    % \ELSE
    % % \IF{any $c_i$ = 0}
    % %         \STATE Algorithm converged to an unfeasible solution. 
    % %     \ELSE
    %         \STATE Algorithm converged to critical point $\boldsymbol{\mu}^* = \boldsymbol{\mu}_t$. 
    %         %to a feasible solution. \\
    %         \textbf{Return} 
    %         %(locally) optimal sampling scheme 
    %         $\boldsymbol{\mu}_t$.
    %     % \ENDIF
    % \ENDIF

%We note that multiple iterations of step \ref{alg:iter_start}--\ref{alg:iter_end} in Algorithm \ref{alg:lopt} may be needed to ensure that a feasible solution is obtained, since in each iteration it is some new instances may achieve $\mu^*_i>1$. 


%In practice, procedures that allow $c_i$ and $\mu_i$ to be zero, or arbitrarily close to zero, tend to produce estimators with unstable performance and should not be used \citep[see, e.g.,][]{Ma2015, Imberg2022b}. We will return to this issue in Section \ref{sec:practical_implementation}.


%We observe from Lemma \ref{lemma:partial_derivatives} that the objective function $\Phi(\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)$ decreases monotonically with increasing values of $\mu_i$. We constrain the optimisation by requiring the expected sample size $n = \sum_{i\in \mathcal D}\mu_i$ to be fixed, restricting the optimisation problem to an \mathprefix{N-1}-dimensional hyperplane in $\mathbb{R}^N$. Hence, we need to balance the contribution from the individual elements $i \in \mathcal D$. The optimality conditions of Proposition \ref{prop:optimality_conditions} characterise the constrained extremum points of the objective function. We show below that D- and L-optimality are convex in $\boldsymbol{\mu}$ and hence that global optimality can be deduced.



%$\mathbf{L}(\boldsymbol{\mu}; \boldsymbol{\theta}_0) = \boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)^{-1/2}$ or $\mathbf{L}(\boldsymbol{\mu}; \boldsymbol{\theta}_0) = \chol(\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)^{-1})$, 


%For a symmetric positive definite matrix $\mathbf{U}$, we let $\mathbf{U}^{1/2}$ denote the matrix square root and $\mathrm{chol}(\mathbf{U})$ the Cholesky factorisation of $\mathbf{U}$, so that $\mathbf{U} = \mathbf{U}^{1/2}\mathbf{U}^{1/2} = \mathrm{chol}(\mathbf{U})\mathrm{chol}(\mathbf{U})\T$. We note that the matrix square root exists, is unique and real-valued whenever $\mathbf{U}$ is positive semi-definite. The Cholesky decomposition exists whenever $\mathbf{U}$ is positive definite.

%Invariance properties are discussed in Section \ref{sec:invariance}. 


%Sometimes the D-optimality criterion is restricted to a subset of parameters or linear combinations of interest, resulting in the so called D$_{\mathrm{A}}$-optimality criterion. The D$_{\mathrm{A}}$-optimality criterion may be addressed by similar means as D-optimality and will therefore not achieve specific attention in this paper. 

%An optimal design $\xi^*$ in a class of experiments $\Xi$ with corresponding consistent estimators $\hat{\boldsymbol{\theta}}_{\xi}$ for an unknown parameter $\boldsymbol{\theta}^*$ is given by 
% \[
% \xi^* = \argmin_{\xi \in \Xi} \Phi(\boldsymbol{\Gamma}_{\xi}),
% \]
% where $\Phi$ is a real-valued function on the set of symmetric positive semi-definite matrices, and $\boldsymbol{\Gamma}_{\xi}$ the covariance matrix of the estimator $\hat{\boldsymbol{\theta}}_{\xi}$. For $\Phi$ to be a sensible objective function for optimal design, one usually requires $\Phi$ to be monotone for Loewner's ordering, i.e., that $\Phi(\boldsymbol{A}) \ge \Phi(\boldsymbol{B})$ every pair of positive semi-definite matrices $\boldsymbol{A}, \boldsymbol{B} \in \boldsymbol{S}_{\!+}^{p \times p}$ such that $\boldsymbol{A} - \boldsymbol{B}$ is positive semi-definite. We note that this is fulfilled for all optimality criteria discussed above. 

%The assumptions include standard ($2+\delta$-bounded) moment conditions on $\mu_i^{-1}S_i\boldsymbol{\psi}_i(\boldsymbol{\theta})\bigr\rvert_{\boldsymbol{\theta} = \boldsymbol{\theta}_0}$, standard conditions on the parameter space (e.g., openness in a neighbourhood of $\boldsymbol{\theta}_0$), and that the empirical risk function $\ell_0(\boldsymbol{\theta})$ is convex and twice differentiable with full-rank Hessian matrix at $\boldsymbol{\theta}_0$. 

%In the context of the examples \ref{list:finite_population_inference}–\ref{list:regression_modelling} presented above, the Hansen-Hurwitz ERM \eqref{eq:thetahat} corresponds to the Hajék estimator $(\sum_i \frac{S_i}{\mu_i})^{-1}\sum_i \frac{S_i\boldsymbol{y}_i}{\mu_i}$ of the vector of finite population means in \ref{list:finite_population_inference}, a weighted (pseudo) maximum likelihood estimator in \ref{list:parametric_density_estimation}, and a weighted quasi-maximum likelihood estimator in \ref{list:regression_modelling} 
% Hence, if $\boldsymbol{\mu}^*$ is L-optimal for $\hat{\boldsymbol{\theta}}_{\!\boldsymbol{\mu}}$, then $\boldsymbol{\mu}^*$ is also L-optimal for $\hat{\boldsymbol{\eta}}_{\!\boldsymbol{\mu}} = \boldsymbol{g}(\hat{\boldsymbol{\theta}}_{\!\boldsymbol{\mu}})$ with $\widetilde{\mathbf{L}} = \mathbf{J}^{-1}_{\!\boldsymbol{g}}(\boldsymbol{\theta}_0)\T\mathbf{L}$.

%Let $\mathcal H$ be a set of non-singular affine transformations $\boldsymbol{h}: (\boldsymbol{x}_i, \boldsymbol{y}_i) \mapsto (\boldsymbol{a} + \boldsymbol{B} \boldsymbol{x}_i, \mathbf{c} + \boldsymbol{D} \boldsymbol{y}_i)$ satisfying the conditions \ref{list:well_defined}--\ref{list:delta_method}, and $\boldsymbol{g}_{\boldsymbol{h}}$ the induced transformation on the parameter space according to \ref{list:induced$_HH}. 


%Invariance properties of optimality criteria and corresponding optimal sampling schemes are discussed below and further in Section \ref{sec:another_look_at_invariance}.
%Indeed, this follows immediately from \eqref{eq:cov_eta}–\eqref{eq:cov_zeta} since the determinant of a matrix product is the product of the determinants, and the factor depending on the design ($\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)$) is unaffected by the transformation.


%in the sense of Proposition \ref{prop:invariance}. 



% A typical situation where transformation- and parameterisation-invariant L-optimality criteria are encountered is when the optimality criterion is defined to capture a comparison or evaluation of specific scientific interest. As an example, consider the problem of estimating the mean difference between two subgroups in the data. An optimal design may in this context be defined using the c-optimality criterion. The group means $\bar y_0, \bar y_1$ may for instance be parameterised as $\bar y_i = \alpha_i = \beta_0 + \delta_i = \gamma_0 + \gamma_1 \times i$, where $i = 0$ or $1$. Clearly, the contrast vector for the c-optimality criterion depends on the choice of parameterisation. 
%The I- and V-optimality criteria are also invariant in this sense.
%The precise relation between the parameterisation and optimality criterion is formalised in Proposition \ref{prop:invariance}. 
%Our primary use of $\Phi_r$-optimality will be to emulate E-optimality using the more tractable $\Phi_r$-optimality criterion. 



%Among the optimality criteria listed in Table \ref{tab:OED}, only D- (and D$_{\mathrm{A}}-)$ optimality and some specific cases of c- and L-optimality are invariant to affine invertible transformations of the data $\{(\boldsymbol{x}_i, \boldsymbol{y}_i)\}_{i \in \mathcal D}$ and one-to-one differentiable transformations of the parameter $\boldsymbol{\theta}$. These properties will be discussed further in Section \ref{sec:invariance} and \ref{sec:another_look_at_invariance}.

% Similarly, consider a non-singular affine transformation $\boldsymbol{h}: (\boldsymbol{x}_i, \boldsymbol{y}_i) \mapsto (\boldsymbol{a} + \boldsymbol{B} \boldsymbol{x}_i, \mathbf{c} + \boldsymbol{D} \boldsymbol{y}_i)$ such that 
% \begin{enumerate}[label = (C\arabic*)]
%     \item $\ell_i(\boldsymbol{\theta}; \boldsymbol{h}(\boldsymbol{x}_i, \boldsymbol{y}_i))$ is defined and finite for all $i \in \mathcal D$,
%     \label{list:well_defined}
%     \item the minimiser of the induced empirical risk $\ell^*_{0, \boldsymbol{h}}(\boldsymbol{\theta}) := \sum_{i \in \mathcal D}\ell(\boldsymbol{\theta}; \boldsymbol{h}(\boldsymbol{x}_i, \boldsymbol{y}_i))$ is given by $\boldsymbol{\zeta}_0 = \boldsymbol{g}_{\boldsymbol{h}}(\boldsymbol{\theta}_0)$, and the corresponding Hansen-Hurwitz empirical risk minimiser for $\boldsymbol{\zeta}_0$ by $\hat{\boldsymbol{\zeta}}_{\!\boldsymbol{\mu}} = \boldsymbol{g}_{\boldsymbol{h}}(\hat{\boldsymbol{\theta}}_{\!\boldsymbol{\mu}})$, where $\boldsymbol{g}_{\boldsymbol{h}}$ is a one-to-one differentiable mapping on the parameter space, and
%     \label{list:induced_HH}
%     \item the covariance matrix of $\hat{\boldsymbol{\zeta}}_{\!\boldsymbol{\mu}}$ is given by 
%     \begin{align}
%         \label{eq:cov_zeta}
%         \COV(\hat{\boldsymbol{\zeta}}_{\!\boldsymbol{\mu}} - \boldsymbol{\zeta}_0)  = \boldsymbol{\Gamma}_{\!\boldsymbol{g}_{\boldsymbol{h}}}\!(\boldsymbol{\mu}; \boldsymbol{\theta}_0) + o(n^{-1}), \quad
%         \boldsymbol{\Gamma}_{\!\boldsymbol{g}_{\boldsymbol{h}}}\!(\boldsymbol{\mu}; \boldsymbol{\theta}_0) = 
%         \mathbf{J}_{\boldsymbol{g}_{\boldsymbol{h}}}\!(\boldsymbol{\theta}_0)
%         \boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0) \mathbf{J}_{\boldsymbol{g}_{\boldsymbol{h}}}\!(\boldsymbol{\mu}; \boldsymbol{\theta}_0)\T,    
%     \end{align}
%     where $\mathbf{J}_{\boldsymbol{g}_{\boldsymbol{h}}}\!(\boldsymbol{\theta})$ is the Jacobian of ${\boldsymbol{g}_{\boldsymbol{h}}}$.
%     \label{list:delta_method}
% \end{enumerate}
% We say that an optimality criterion and corresponding optimal sampling scheme is invariant under an affine transformation $\boldsymbol{h}$, satisfying the conditions \ref{list:well_defined}--\ref{list:delta_method}, if the optimal sampling schemes for $\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)$ and $\boldsymbol{\Gamma}_{\!\boldsymbol{g}_{\boldsymbol{h}}}\!(\boldsymbol{\mu}; \boldsymbol{\theta}_0)$ are equal. 



% The conditions \ref{list:well_defined}--\ref{list:delta_method} on the affine transformation $\boldsymbol{h}$ are needed to ensure that the induced empirical risk is well-defined, and that the statistical properties of the estimator are qualitatively unchanged by the data-transformation. 
% An example of a model- and transformation-pair that may violate these assumptions is a location shift in a variable that is modelled by a probability distribution with support on the positive real line. 
% Another example is an affine transformation of the data in a regression model that does obey the principle of strong hierarchy, i.e., does not include all lower-order terms in a polynomial regression model, or does not include all main effects and lower-order interactions in an interaction model (ref). 
% Phrased differently, affine transformations that satisfy \ref{list:well_defined}--\ref{list:delta_method} are transformations that produce mathematically equivalent models. This is a prerequisite for invariance of the optimal design under transformations of the data. 
%For most models there is a natural class of transformations that preserve the principle of equivariance, and for which invariance of 
%Note that \ref{list:induced_HH} that in this case we may have two alter  is a consequence of the delta method as in this case we have two alternative and possible conflc and states that the transformation of the data should result in a transformations of the parameter such that the covariance structure is preserved, and the delta method hold.  the statistical properties are equivariant and the delta method preserve equivariance of the parameters transformation should be such that the delta methodis a consequence of the delta method. It states that our inference from $\hat{\boldsymbol{\zeta}}_{\!\boldsymbol{\mu}}$ should be the same irrespective of whether we evaluate the properties of $\hat{\boldsymbol{\zeta}}_{\!\boldsymbol{\mu}}$ by the delta method or using the theoretical machinery of Section \ref{sec:approximate_covariance_matrix}. 

%When \ref{list:well_defined}--\ref{list:delta_method} are not fulfilled, the statistical properties of the estimator are qualitatively affected by the transformation, which violoates the principle of equivariance and makes a 
%Indeed, the empirical risk may not be   through the origin, As a counter-example, consider the case where $y_i$ is a positive variable modelled by a probability distribution with support on the positive real line. Such models are in general sensitive to location shifts in the data, and \ref{list:well_defined} may be violated if applying an arbitrary location shift $y_i \mapsto y_i + a$, $a>0$ when $y_i$ is modelled by a . Such models are in general sensitive to location shifts in the data. Another example is regression through the origin, where the assumption \ref{list:delta_method} may be violated if applying an by an arbitrary affine transformation $\boldsymbol{h}: (\boldsymbol{x}_i, \boldsymbol{y}_i) \mapsto (\boldsymbol{a} + \boldsymbol{B} \boldsymbol{x}_i, \mathbf{c} + \boldsymbol{D} \boldsymbol{y}_i)$ with $\boldsymbol{a} \ne \boldsymbol{0}$ or $\boldsymbol{c} \ne \boldsymbol{0}$. 
%Phrased differently, affine transformations that satisfy \ref{list:well_defined}--\ref{list:delta_method} are transformations that produce mathematically equivalent models. 
%Moreover, these are assumptions on the model and rather than conditions on the the data. Examples of transformation would be violated if, e.g., applying an affine transformation %These assumptions hold true in most cases where the transformation preserves the domain of the data
%The last three conditions are properties of equivariance: the full-data parameter and estimator $\boldsymbol{\theta}_0$ should be affected equally by the transformation, and the delta method should hold. That is, we should achieve the same expression for the approximate variance of $\boldsymbol{g}_{\boldsymbol{h}}(\hat{\boldsymbol{\theta}}_{\!\boldsymbol{\mu}})$ irrespective of whether it is derived directly from the induced empirical risk, or by the delta method for $\boldsymbol{g}_{\boldsymbol{h}}(\hat{\boldsymbol{\theta}}_{\!\boldsymbol{\mu}})$. We cannot expect to obtain transformation-invariance unless such a restriction is made. As an example, consider regression through the origin. In this case $\mathcal H$ is the space of non-singular linear transformations. Extending $\mathcal H$ to include all non-singular affine transformations is not possible, since such transformations do not produce mathematically equivalent models when the regression line is forced through the origin. In this example, the constraints on $\mathcal H$ are induced by the model. There may also exist natural constraints on the data that preclude consideration of certain transformations of the data. For instance, arbitrary affine transformations may not be appropriate for variables living on a restricted domain, e.g., on the positive real line. 



%let $\boldsymbol{g}_{\boldsymbol{h}}(\boldsymbol{\theta}_0) = \argmin_{\boldsymbol{\theta} \in \boldsymbol{\Omega}} \ell^*_{0, \boldsymbol{h}}(\boldsymbol{\theta})$ be the minimiser of the induced empirical risk $\ell^*_{0, \boldsymbol{h}}(\boldsymbol{\theta}) := \sum_{i \in \mathcal D}\ell(\boldsymbol{h}(\boldsymbol{x}_i, \boldsymbol{y}_i); \boldsymbol{\theta})$. Let $\mathbf{X}, \mathbf{Y}$ be the matrices with rows $\boldsymbol{x}_i\T, \boldsymbol{y}_i\T$, and $\mathbf{X}_{\!\boldsymbol{h}}, \mathbf{Y}_{\!\boldsymbol{h}}$ the corresponding matrices after the transformation $\boldsymbol{h}$. 



% \begin{proposition}[Invariant L-optimal sampling schemes] %%\hspace{1cm} \\
% \label{prop:invariance}
% Let $\boldsymbol{g}: \boldsymbol{\Omega} \to \boldsymbol{\Omega}$ be a one-to-one differentiable transformation on the parameter space and $\boldsymbol{J}_{\!\boldsymbol{g}}(\boldsymbol{\theta})$ the Jacobian of $\boldsymbol{g}$. Let $\boldsymbol{h}: (\boldsymbol{x}_i, \boldsymbol{y}_i) \mapsto (\boldsymbol{a} + \boldsymbol{B} \boldsymbol{x}_i, \mathbf{c} + \boldsymbol{D} \boldsymbol{y}_i)$ be a non-singular affine transformation of the data satisfying \ref{list:well_defined}–\ref{list:delta_method}, and $\boldsymbol{g}_{\boldsymbol{h}}$ the induced transformation on the parameter space according to \ref{list:induced_HH}. Let $\mathbf{X}, \mathbf{Y}$ be the matrices with rows $\boldsymbol{x}_i\T, \boldsymbol{y}_i\T$, and $\mathbf{X}_{\!\boldsymbol{h}}, \mathbf{Y}_{\!\boldsymbol{h}}$ the matrices with rows $(\boldsymbol{a} + \boldsymbol{B} \boldsymbol{x}_i)\T, (\mathbf{c} + \boldsymbol{D} \boldsymbol{y}_i)\T$. Consider a linear optimality criterion with respect to an non-zero $d \times m$ matrix $\mathbf{L}$ such that 
%     \begin{enumerate}[label = (A\arabic*)]
%         \item $\mathbf{L} = \mathbf{L}(\boldsymbol{g}(\boldsymbol{\theta}_0))$ is a function of the transformation $\boldsymbol{g}$ such that $\mathbf{L}(\boldsymbol{g}(\boldsymbol{\theta}_0)) = \boldsymbol{J}^{-1}_{\!\boldsymbol{g}}(\boldsymbol{\theta}_0)\T\mathbf{L}(\boldsymbol{\theta}_0)$, 
%         \label{ass:parameterisation_invariance}
%         \item $\mathbf{L} = \mathbf{L}(\mathbf{X}_{\!\boldsymbol{h}}, \mathbf{Y}_{\!\boldsymbol{h}})$ is a function of $\boldsymbol{h}$ such that $\mathbf{L}(\mathbf{X}_{\!\boldsymbol{h}}, \mathbf{Y}_{\!\boldsymbol{h}}) = k \boldsymbol{J}^{-1}_{\!\boldsymbol{g}_{\boldsymbol{h}}}(\boldsymbol{\theta}_0)\T\mathbf{L}(\mathbf{X}, \mathbf{Y})$,
%         \label{ass:transformation_invariance}
%     \end{enumerate}
%     where $k\ne 0$ is an arbitrary constant.
%     %, i.e., the $d \times d$ matrix with rows $\nabla\T_{\!\boldsymbol{\theta}}g_k(\boldsymbol{\theta}), k = 1, \ldots, d$. 
%     Then the following holds:
%     \begin{enumerate}[label = \alph*)]
%         \item \ref{ass:parameterisation_invariance} implies that the L-optimal sampling scheme for $\mathbf{L} = \mathbf{L}(\boldsymbol{g}(\boldsymbol{\theta}_0))$ is invariant under the re-parameterisation $\boldsymbol{g}: \boldsymbol{\theta} \mapsto \boldsymbol{\eta}$.
%         \label{prop:parameterisation_invariance}
%         \item \ref{ass:transformation_invariance} implies that the L-optimal sampling scheme for $\mathbf{L} = \mathbf{L}(\mathbf{X}_{\!\boldsymbol{h}}, \mathbf{Y}_{\!\boldsymbol{h}})$ is invariant under the affine transformation $\boldsymbol{h}: (\boldsymbol{x}_i, \boldsymbol{y}_i) \mapsto (\boldsymbol{a} + \boldsymbol{B} \boldsymbol{x}_i, \mathbf{c} + \boldsymbol{D} \boldsymbol{y}_i)$.
%         \label{prop:transformation_invariance}
%         \item If, in addition, the gradients $\{\boldsymbol{\psi}_i(\boldsymbol{\theta}_0)\}_{i \in \mathcal D}$ span $\mathbb{R}^d$, then \ref{ass:parameterisation_invariance} and \ref{ass:transformation_invariance} also also necessary conditions for parameterisation- and transformation-invariance. 
%     \end{enumerate}
% \end{proposition}



%We note that the optimality criteria discussed in Section \ref{sec:d_star_examples} correspond to L-optimality with a coefficient matrix $\mathbf{L}$ that depends on the Hessian matrix $\mathbf{H}(\boldsymbol{\theta}_0)$ and outer products $\boldsymbol{\psi}_i(\boldsymbol{\theta}_0)\boldsymbol{\psi}_i(\boldsymbol{\theta}_0)\T$ in a very specific manner. This is crucial to achieve transformation- and parameterisation invariance. Indeed, we show in Proposition \ref{prop:invariance} that L-optimality with $\mathbf{L} = \mathbf{H}(\boldsymbol{\theta})^{1/2}$ or $\mathbf{L} = \mathbf{H}(\boldsymbol{\theta})\mathbf{V}(\boldsymbol{\theta})^{-1/2}$ yield sampling schemes with desirable invariance properties, and moreover span the space of such invariant L-optimal designs.

%The result above shows that any invariant L-optimality criterion is in direct correspondence with the Hessian matrix $\mathbf{H}(\boldsymbol{\theta}_0)$ and gradient covariance matrix $\mathbf{V}(\boldsymbol{\theta}_0)$. Indeed, for an invariant L-optimal sampling scheme, any data transformation or change in parameterisation must be accompanied by an equivalent change in the L-optimality criterion according to Proposition \ref{prop:invariance}. Furthermore, any such change under the conditions of Proposition \ref{prop:invariance} induces an equivalent change in $\mathbf{H}(\boldsymbol{\theta}_0)^{1/2}$ and $\mathbf{H}(\boldsymbol{\theta}_0)\mathbf{V}(\boldsymbol{\theta})^{-1/2}$. To obtain an invariant all-purpose  L-optimality criterion, we may take $\widetilde{\mathbf{L}} = \mathbf{I}_{d \times d}$ in Proposition \ref{prop:invariance}, corresponding to L-optimality with $\mathbf{L} = \widetilde{\mathbf{H}}(\boldsymbol{\theta}_0)^{1/2}$, $\mathbf{L} = \mathbf{H}(\boldsymbol{\theta}_0)^{1/2}$ and $\mathbf{L} = \mathbf{H}(\boldsymbol{\theta}_0)\mathbf{V}(\boldsymbol{\theta})^{-1/2}$, respectively. According to the results of Section \ref{sec:d_star_examples}, this corresponds to minimising the expected Kullback-Leibler divergence, empirical risk distance, and/or Mahalanobis distance from the estimator $\hat{\boldsymbol{\theta}}_{\!\boldsymbol{\mu}}$ to the full-data parameter $\boldsymbol{\theta}_0$.

%Its inverse measures, on a relative scale, how many more observations that are needed with the sampling scheme $\boldsymbol{\mu}$ to reach the same level of performance as the optimal sampling scheme. 
%$\Phi$-optimal sampling scheme $\boldsymbol{\mu}^*$ to reach the same level of performance for the objective function $\Phi$ as with the sampling scheme $\boldsymbol{\mu}$. 
%Phrased differently, it gives the extent to which the sampling scheme $\boldsymbol{\mu}$ reaches the minimum  information $\Phi(\boldsymbol{\Gamma}(\boldsymbol{\mu}^*; \boldsymbol{\theta}_0))$. 

%We consider A-, D-, and E-optimality, and $\Phi_r$-optimality with $p=0.5$, $p=5$, and $p=10$. We also consider L-optimality with $\mathbf{L} = \mathbf{H}(\boldsymbol{\theta}_0)^{1/2}$ and $\mathbf{L}= \mathbf{H}(\boldsymbol{\theta}_0)\mathbf{V}(\boldsymbol{\theta}_0)^{-1/2}$, where $\mathbf{V}(\boldsymbol{\theta}) = \sum_{i \in \mathcal D}\boldsymbol{\psi}_i(\boldsymbol{\theta})\boldsymbol{\psi}_i(\boldsymbol{\theta})\T$. The L-optimality criterion with $\mathbf{H}(\boldsymbol{\theta}_0)^{1/2}$ minimises the generalisation error of the estimator $\hat{\boldsymbol{\theta}}_{\!\boldsymbol{\mu}}$, in the sense of minimising the expected empirical distance from $\boldsymbol{\theta}_0$ to $\hat{\boldsymbol{\theta}}_{\!\boldsymbol{\mu}}$. This is related to the V-optimality criterion sometimes used in traditional optimal design (ref). The D-optimality criterion and the two L-optimality criteria are invariant to the parameterisation of the model and to non-singular affine transformation of the model matrix $\mathbf{X}$.
%In addition to the optimality criteria listed in Section \ref{sec:background}, we also include the c-optimality criterion with $\mathbf{c} = (1,0)\T$ and $\mathbf{c} = (0,1)\T$. 
%, and the L-optimality criterion with $\mathbf{L} = \mathbf{L}_z$, where $\mathbf{L}_z$ is the matrix with columns $(1, z_{j/100})\T, j = 1, \ldots, 99$, and $z_{\alpha}$ the $\alpha$-quantile of the standard normal distribution. This L-optimality criterion minimises the average variance of the estimated percentiles of the log impact speed from the fitted log-normal distribution. 


% We consider A-, D-, and E-optimality; c-optimality with $\mathbf{c} = (1, 0)\T$ and $\mathbf{c} = (0, 1)\T$; $\Phi_r$-optimality with $r=0.5$, $r=5$, and $r=10$. We also consider L-optimality with $\mathbf{L} = \mathbf{H}(\boldsymbol{\theta}_0)^{1/2}$, $\mathbf{L}= \mathbf{H}(\boldsymbol{\theta}_0)\mathbf{V}(\boldsymbol{\theta}_0)^{-1/2}$, and $\mathbf{L} = \mathbf{L}_z$, where $\mathbf{V}(\boldsymbol{\theta}) = \sum_{i \in \mathcal D}\boldsymbol{\psi}_i(\boldsymbol{\theta})\boldsymbol{\psi}_i(\boldsymbol{\theta})\T$, $\mathbf{L}_z$ the matrix with columns $(1, z_{j/100})\T, j = 1, \ldots, 99$, and $z_{\alpha}$ the $\alpha$-quantile of the standard normal distribution. The L-optimality criterion with $\mathbf{L} = \mathbf{L}_z$ is included here to minimise the average variance of the estimated percentiles of the fitted log-normal distribution. According to the results of Section \ref{sec:dist} the L-optimality criterion with $\mathbf{L} = \mathbf{H}(\boldsymbol{\theta}_0)^{1/2} = \widetilde{\mathbf{H}}(\boldsymbol{\theta}_0)^{1/2}$ minimises expected distance of $\hat{\boldsymbol{\theta}}_{\!\boldsymbol{\mu}}$ from the full-data parameter $\boldsymbol{\theta}_0$ in the Kullback-Leibler sense, as illustrated in Figure \ref{fig:KL}. The D-optimality criterion and L-optimality criteria with $\mathbf{L} = \mathbf{H}(\boldsymbol{\theta}_0)^{1/2}$ and $\mathbf{L}= \mathbf{H}(\boldsymbol{\theta}_0)\mathbf{V}(\boldsymbol{\theta}_0)^{-1/2}$ are invariant to linear transformations of the data and to the parameterisation of the model.



% \begin{figure}[!htb]
%     \centering
%     \includegraphics[scale = 1]{Figures/Figure1.png}
%     \caption{Fitted log-normal densities for the baseline impact speed distribution on the full dataset and on 10 randomly selected subsets of size $n=100$. The L-optimality criterion with $\mathbf{L} = \widetilde{\mathbf{H}}(\boldsymbol{\theta}_0)^{1/2}$ minimises the expected distance of the dashed curves to the solid curve with respect to the Kullback-Leibler divergence.}
%     \label{fig:KL}
% \end{figure}


%In this case auxiliary information for $\boldsymbol{y}_i$ is available through the known scenario generation parameters, i.e. the case identifier, off-road glance duration, and maximal deceleration. 
%Moreover, we only need to specify the first two moments of $\mathbf{Y}_i$. 
%If we once again consider the case where all observation weights $w_i$ are equal, the inner term of \eqref{eq:opt_fps} is equal to the squared Mahalanobis distance of the predicted response vector from the overall mean, plus an additional term that accounts for the uncertainty in the prediction relatively to the sample covariance variance of $\{\boldsymbol{y}_i\}_{i=1}^N$. 

% \subsection{Concluding remarks on the application and examples}
% \label{sec:remarks}

% In Section \ref{sec:parametric_density_estimation}–\ref{sec:finite_population_inference} we have presented an analytical comparison of optimality criteria for different aspects of virtual safety assessment of an advanced driver assistance system. Moreover, in \eqref{eq:mu_density_estimation}, \eqref{eq:leverage_sampling} and \eqref{eq:opt_fps} we have presented formulas for optimal sampling schemes with respect to the anticipated covariance matrix for selected optimality criteria. Optimal sampling schemes for other optimality criteria may be derived by similar means.  Auxiliary variables are in this application available through the known scenario parameters, i.e., case identifier, maximal deceleration, and off-road glance durations. 



% We note that the optimal sampling schemes in \eqref{eq:mu_density_estimation}, \eqref{eq:leverage_sampling} and \eqref{eq:opt_fps} require a preliminary estimate $\tilde{\boldsymbol{\theta}}_0$ of the full-data parameter $\boldsymbol{\theta}_0$, and additionally a model $f(\boldsymbol{y}|\boldsymbol{z})$ for the conditional distribution of the outcome $\boldsymbol{y}_i$ given the auxiliary variables $\boldsymbol{z}_i$. This can be handled using sequential optimal design as outlined in Section \ref{sec:multistage_sampling}.
% %See, e.g., \citet{Imberg2020, Imberg2022a} and \citet{Imberg2022b} for examples and applications with practical implementations of such algorithms. 
% See \citet{Imberg2022b} for a practical implementation for the c-optimality criterion in this specific application. 


%We note that these two expressions coincide if the A-optimality criterion is applied after a change of variables $\boldsymbol{y}_i \mapsto \mathbf{V}(\boldsymbol{\theta}_0)^{-1/2}\boldsymbol{y}_i$, where $\mathbf{V}(\boldsymbol{\theta}_0) = \sum_{i \in \mathcal D} \boldsymbol{\psi}_i(\boldsymbol{\theta}_0)\boldsymbol{\psi}_i(\boldsymbol{\theta}_0)^T$.
%If all observation weights $w_i$ are equal, this corresponds to an orthogonalisation of the data.
%change to $ In this case, we recognise \eqref{eq:ci_fps} as the squared Mahalanobis distance of the response vector $\boldsymbol{y}_i$ from the overall mean $\boldsymbol{\theta}_0$. Similarly, the transformation $\boldsymbol{y}_i \mapsto \mathbf{V}(\boldsymbol{\theta}_0)^{-1/2}\boldsymbol{y}_i$ will then correspond to orthogonalisation of the data.


%evaluated at a preliminary estimate $\tilde{\boldsymbol{\theta}}_0$ of $\boldsymbol{\theta}_0$, and normalised so that $\sum_{i=1}^N \mu_i = n$. 


%We note that this result differs from \citet{Imberg2020} where $\Var(Y_i - p_i(\boldsymbol{\theta}_0)) = p_i(\boldsymbol{\theta}_0)(1-p_i(\boldsymbol{\theta}_0))$ was assumed, and hence a sampling scheme with $\mu \propto \sqrt{h_{ii}}$ was used. See \citet{Ma2020} for a related discussion for ordinary linear models. As before, we note that the sampling scheme \eqref{eq:leverage_sampling} is guaranteed to produce strictly positive sampling probabilities as long as the predictions $p_i(\boldsymbol{\theta}_0)$ are bounded away from $0$ and $1$.


% \nonumber
    % c_i & = (y_i - p_i(\boldsymbol{\theta}_0))^2 \boldsymbol{x}_i\T \mathbf{H}(\boldsymbol{\theta}_0)^{-2}\boldsymbol{x}_i, \quad \text{(A-optimality)} \\

%We note that these two expressions coincide if the A-optimality criterion is applied after a change of variables $\mathbf{X} \mapsto \tilde{\mathbf{X}} := \mathbf{X}\mathbf{H}(\boldsymbol{\theta}_0)^{-1/2}$. For ordinary least squares regression, $\mathbf{W}(\boldsymbol{\theta}_0) \propto \mathbf{I}_{N\times N}$ and d$^*_{\mathrm{ER}}$-optimality corresponds to A-optimality after a change to orthogonal coordinates, i.e., such that the columns of the resulting data matrix $\tilde{\mathbf{X}}$ are uncorrelated with unit variance. 

%In addition to the optimality criteria listed in Section \ref{sec:background}, we also include the c-optimality criterion with $\mathbf{c} = (1, 0, 0)\T$, $\mathbf{c} = (0, 1, 0)\T$, and $\mathbf{c} = (0, 0, 1)\T$
%, and the L-optimality criterion with $\mathbf{L} = \mathbf{L}_{S_{wY}}$, where $\mathbf{L}_{S_{wY}}\mathbf{L}_{S_{wY}}\T = \sum_{i=1}^N w_i(\boldsymbol{y}_i - \boldsymbol{\theta}_0)(\boldsymbol{y}_i - \boldsymbol{\theta}_0)\T$ is (proportional to) the weighted sample covariance matrix of $\{\boldsymbol{y}_i\}_{i=1}^N$. We note that $\mathrm{L}_{S_{wY}}$-optimality coincides with d$^*_{\mathrm{S}}$-optimality when all observation weights $w_i$ are equal. In this case it also coincides with A-optimality if the response matrix $\mathbf{Y}$ (i.e., the matrix with rows $\boldsymbol{y}_i^T$) has orthogonal columns. 
%In contrast, the D-, d$^*_{\mathrm{S}}$-, and L-optimality criterion with $\mathbf{L} = \mathbf{S}^2_{w}(\mathbf{Y})^{-1/2}$ are invariant to arbitrary non-singular affine transformations of the data. 
%Also note that when all observations weights $w_i$ are equal, the 
%d$^*_{\mathrm{S}}$-optimality criterion and L-optimality criterion with $\mathbf{L} = \mathbf{S}^2_{w}(\mathbf{Y})^{-1/2}$ are identical. 


% latex table generated in R 4.2.2 by xtable 1.8-4 package
% Mon Feb 20 08:40:57 2023
\begin{table}[htb!]
\centering
\caption{Evaluation of sampling schemes for estimating the safety benefits from an automatic emergency braking system compared to baseline manual driving, in terms of mean impact speed reduction, mean injury risk reduction, and crash avoidance rate. \textit{eff = relative efficiency.}} 
\label{tab:finite_population_inference}
\begin{tabular}{p{2.75cm}R{3.125cm}R{0.9cm}R{1.5cm}R{1.5cm}R{1.5cm}R{0.9cm}R{0.9cm}}
  % \multicolumn{2}{l}{} & 
  % \multicolumn{6}{c}{Relative efficiency} \\
  % \cmidrule{3-8} 
Optimality criterion & No. iterations needed for convergence & A-eff & c$_{(1,0,0)}$-eff & c$_{(0,1,0)}$-eff & c$_{(0,0,1)}$-eff & D-eff & E-eff \\ 
  \hline
A & 1 & \textbf{1.00} & \textbf{1.00} & 0.36 & 0.25 & 0.46 & \textbf{1.00} \\ 
  c, $\mathbf{c} = (1, 0, 0)\T$ & 1 & 0.98 & \textbf{1.00} & 0.05 & 0.04 & 0.20 & \textbf{1.00} \\ 
  c, $\mathbf{c} = (0, 1, 0)\T$ & 1 & 0.12 & 0.12 & \textbf{1.00} & 0.11 & 0.22 & 0.12 \\ 
  c, $\mathbf{c} = (0, 0, 1)\T$ & 1 & 0.41 & 0.41 & 0.50 & \textbf{1.00} & 0.70 & 0.41 \\ 
  D & 2 & 0.67 & 0.67 & 0.77 & 0.81 &\textbf{ 1.00} & 0.67 \\ 
  E & 2 & 0.99 & \textbf{1.00} & 0.07 & 0.06 & 0.22 & \textbf{1.00} \\ 
  d$^*_{\mathrm{ER}}$ & 1 & \textbf{1.00} & \textbf{1.00} & 0.36 & 0.25 & 0.46 & \textbf{1.00} \\ 
  d$^*_{\mathrm{S}}$ & 1 & 0.73 & 0.72 & 0.77 & 0.77 & 0.99 & 0.72 \\ 
  %$\mathrm{L}_{S_{wY}}$ & 1 & 0.76 & 0.76 & 0.75 & 0.79 & 0.97 & 0.76 \\ 
  $\Phi_{0.5}$ & 2 & 0.99 & 0.99 & 0.46 & 0.38 & 0.58 & 0.99 \\ 
  $\Phi_5$ & 2 & 0.99 & \textbf{1.00} & 0.07 & 0.06 & 0.22 & \textbf{1.00} \\ 
  $\Phi_{10}$ & 2 & 0.99 & \textbf{1.00} & 0.07 & 0.06 & 0.22 & \textbf{1.00} \\ 
   \hline   
  %\multicolumn{8}{p{16cm}}{$^*$Number of iterations needed for convergence with the iterative L-approximation algorithm (Algorithm \ref{alg:linearisation}).} \\
  %\newline 
  %$^{\dagger}$The relative efficiency was calculated as the value of the objective function relatively to the optimal value. The objective function of the D-optimality criterion was here defined as $\det( \boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0))^{1/d}$. \newline
  %c$_{xyz}$: c-optimality with $\mathbf{c} = (x, y, z)\T$.} \\
  %d$^*_{\mathrm{ER}}$: L-optimality with $\mathbf{L} = \mathbf{H}(\boldsymbol{\theta}_0)^{1/2}$. 
  %d$^*_{\mathrm{S}}$: L-optimality with $\mathbf{L} = \mathbf{H}(\boldsymbol{\theta}_0)\mathbf{V}(\boldsymbol{\theta}_0)^{-1/2}$. See Section \ref{sec:d_star_examples} for details.} \\
  %$\mathrm{L}_{S_{wY}}$: L-optimality with $\mathbf{L} = \mathbf{L}_{S_{wY}}$, and $\mathbf{L}_{S_{wY}}\mathbf{L}_{S_{wY}}\T = \sum_{i=1}^N w_i(\boldsymbol{y}_i - \boldsymbol{\theta}_0)(\boldsymbol{y}_i - \boldsymbol{\theta}_0)\T$.} \\
  %\hline
  \end{tabular}
\end{table}


% latex table generated in R 4.2.2 by xtable 1.8-4 package
% Mon Feb 20 08:33:13 2023
\begin{table}[htb!]
\centering
\caption{Evaluation of sampling schemes and optimality criteria for estimating the baseline impact speed response surface, as a function of the off-road glance duration and maximal deceleration during braking. \textit{eff = relative efficiency.}} 
\label{tab:impact_speed_response_surface}
\begin{tabular}{p{2.75cm}R{3.125cm}R{1.5cm}R{1.5cm}R{1.5cm}R{1.5cm}R{1.5cm}}
  % \multicolumn{2}{l}{} & 
  % \multicolumn{5}{c}{Relative efficiency} \\
  % \cmidrule{3-7}
  Optimality criterion & No. iterations needed for convergence & A-eff & D-eff & d$^*_{\mathrm{ER}}$-eff & d$^*_{\mathrm{S}}$-eff & $\Phi_{0.5}$-eff \\ 
  \hline
  A & 1 & \textbf{1.00} & 0.65 & 0.54 & 0.49 & 0.95 \\ 
  D & 4 & 0.63 & \textbf{1.00} & 0.93 & 0.95 & 0.81 \\ 
  d$^*_{\mathrm{ER}}$ & 1 & 0.63 & 0.95 & \textbf{1.00} & 0.94 & 0.79 \\ 
  d$^*_{\mathrm{S}}$ & 1 & 0.57 & 0.97 & 0.94 & \textbf{1.00} & 0.75 \\ 
  E & Did not converge &  &  &  &  &  \\ 
  $\Phi_{0.5}$ & 2 & 0.94 & 0.84 & 0.76 & 0.72 & \textbf{1.00} \\ 
  $\Phi_{0.5}$ & Did not converge &  &  &  &  &  \\ 
  $\Phi_{10}$ & Did not converge &  &  &  &  &  \\ \hline   
  %\multicolumn{7}{R{16cm}}{\textit{eff = relative efficiency.}}%\\\hline
  %$^*$Number of iterations needed for convergence with the iterative L-approximation algorithm (Algorithm \ref{alg:linearisation}).}\\
  %\newline 
  %$^{\dagger}$The relative efficiency was calculated as the value of the objective function relatively to the optimal value. The objective function of the D-optimality criterion was here defined as $\det( \boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0))^{1/d}$. \newline
  %d$^*_{\mathrm{ER}}$: L-optimality with $\mathbf{L} = \mathbf{H}(\boldsymbol{\theta}_0)^{1/2}$.  
  %d$^*_{\mathrm{S}}$: L-optimality with $\mathbf{L} = \mathbf{H}(\boldsymbol{\theta}_0)\mathbf{V}(\boldsymbol{\theta}_0)^{-1/2}$. See section \ref{sec:d_star_examples} for details.} \\ \hline
\end{tabular}
\end{table}

\captionsetup[table]{skip=5pt}



% latex table generated in R 4.2.2 by xtable 1.8-4 package
% Mon Feb 20 08:58:06 2023
\begin{table}[htb!]
\centering
\caption{Evaluation of sampling schemes and optimality criteria for estimating the baseline impact speed distribution, assuming a log-normal model. \textit{eff = relative efficiency.}} 
\label{tab:baseline_impact_speed}
\begin{tabular}{p{2.75cm}R{3.125cm}R{1.1cm}R{1.3cm}R{1.3cm}R{1.1cm}R{1.2cm}R{1.2cm}}
  %\multicolumn{2}{l}{} & 
  %\multicolumn{6}{c}{Relative efficiency} \\
  %\cmidrule{3-8}
Optimality criterion & No. iterations needed for convergence & A-eff & c$_{(1,0)}$-eff & c$_{(0, 1)}$-eff & D-eff & d$^*_{\mathrm{ER}}$-eff & $\Phi_5$-eff \\ 
  \hline
A & 1 & \textbf{1.00} & 0.90 & 0.76 & 0.99 & 0.99 & 0.96 \\ 
  c, $\mathbf{c} = (1, 0)\T$ & 1 & 0.14 & \textbf{1.00} & 0.04 & 0.24 & 0.10 & 0.09 \\ 
  c, $\mathbf{c} = (1, 0)\T$ & 1 & 0.27 & 0.16 & \textbf{1.00} & 0.47 & 0.34 & 0.19 \\ 
  D & 3 & 0.98 & 0.86 & 0.79 & \textbf{1.00} & 0.98 & 0.90 \\ 
  d$^*_{\mathrm{ER}}$ & 1 & 0.99 & 0.84 & 0.83 & 0.99 & \textbf{1.00} & 0.92 \\ 
  d$^*_{\mathrm{S}}$ & 1 & 0.97 & 0.84 & 0.79 & 0.96 & 0.98 & 0.94 \\ 
  E & Did not converge &  &  &  &  &  &  \\ 
 % L$_z$ & 1 & \textbf{1.00} & 0.91 & 0.75 & 0.99 & 0.98 & \textbf{1.00} & 0.96 \\ 
  $\Phi_{0.5}$ & 2 & \textbf{1.00} & 0.89 & 0.77 & \textbf{1.00} & 0.99  & 0.93 \\ 
  $\Phi_5$ & 43 & 0.96 & 0.93 & 0.64 & 0.91 & 0.91 &\textbf{1.00} \\ 
  $\Phi_{10}$ & Did not converge &  &  &  &  &  &  \\ \hline
  %\multicolumn{8}{p{16cm}}{$^*$Number of iterations needed for convergence with the iterative L-approximation algorithm (Algorithm \ref{alg:linearisation}).}\\
  %\newline 
  % $^{\dagger}$The relative efficiency of a sampling scheme $\boldsymbol{\mu}$ with respect to an optimality criterion $\Phi$ was defined as $\Phi(\boldsymbol{\Gamma}(\boldsymbol{\mu}^*; \boldsymbol{\theta}_0)) / \Phi(\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0))$, where $\boldsymbol{\mu}^*$ is the corresponding $\Phi$-optimal sampling scheme. The objective function of the D-optimality criterion was defined as $\det(\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0))^{1/d}$. \newline
  %c$_{10}$: c-optimality with $\mathbf{c} = (1, 0)\T$. 
  %c$_{01}$: c-optimality with $\mathbf{c} = (0, 1)\T$. \newline
  %d$^*_{\mathrm{ER}}$: L-optimality with $\mathbf{L} = \mathbf{H}(\boldsymbol{\theta}_0)^{1/2}$.
  %d$^*_{\mathrm{S}}$: L-optimality with $\mathbf{L} = \mathbf{H}(\boldsymbol{\theta}_0)\mathbf{V}(\boldsymbol{\theta}_0)^{-1/2}$. See Section \ref{sec:d_star_examples} for details. \newline 
  %L$_z$: L-optimality with $\mathbf{L} = \mathbf{L}_z$, where $\mathbf{L}_z$ is the matrix with columns $(1, z_{j/100})\T, j = 1, \ldots, 99$, and $z_{\alpha}$ the $\alpha$-quantile of a standard normal distribution.} \\ \hline
  %\hline
\end{tabular}
\end{table}

% :
    % \begin{enumerate}[label = \alph*)]
    %     \item The d$^*$-optimality criterion is invariant  L-optimal sampling scheme $\boldsymbol{\mu}^*$ is invariant to the parameterisation of the model if and only if $\mathbf{L} = \mathbf{L}(\boldsymbol{\theta}_0)$ is a function of the parameter $\boldsymbol{\theta}_0$ such that
    %     $
    %     \mathbf{L}(\boldsymbol{\theta}_0) =
    %     \mathbf{H}(\boldsymbol{\theta}_0)^{1/2}
    %     \widetilde{\mathbf{L}},
    %     $
    %     where $\widetilde{\mathbf{L}}$ does not depend on $\boldsymbol{\theta}_0$.   \label{prop:invariance_a}
    %     \item If, for every transformation $\boldsymbol{h} \in \mathcal H$, the Hessian of the induced empirical risk $\ell_{0, \boldsymbol{h}}(\boldsymbol{\theta}) = \sum_{i\in \mathcal D} \ell(\boldsymbol{\theta}; \boldsymbol{h}(\boldsymbol{x}_i, \boldsymbol{y}_i))$ is given by $\mathbf{J}_{\boldsymbol{g}_{\boldsymbol{h}}}\!(\boldsymbol{\theta}_0)
    %     \mathbf{H}(\boldsymbol{\theta}_0) \mathbf{J}_{\boldsymbol{g}_{\boldsymbol{h}}}\!(\boldsymbol{\mu}; \boldsymbol{\theta}_0)\T$, then (\ref{prop:invariance_a} also holds for invariance to data transformations in $\mathcal H$. \label{prop:invariance_b}
    %     \item An L-optimal sampling scheme $\boldsymbol{\mu}^*$ is invariant to the parameterisation of the model and to non-singular affine transformations of the data if and only if $\mathbf{L} = \mathbf{L}(\boldsymbol{\theta}_0)$ is a function of the parameter $\boldsymbol{\theta}_0$ such that
    %     $
    %     \mathbf{L}(\boldsymbol{\theta}_0) =
    %     \mathbf{H}(\boldsymbol{\theta}_0)
    %     \mathbf{V}(\boldsymbol{\theta}_0)^{-1/2}
    %     \widetilde{\mathbf{L}},
    %     $
    %     where $\widetilde{\mathbf{L}}$ does not depend on $\boldsymbol{\theta}_0$.
    %     \label{prop:invariance_c}
    % \end{enumerate}
    
    \subsection{Invariance properties}
\label{sec:invariance}

A property that is often desirable of an optimal design, is invariance to the parameterisation of the model and under non-singular affine transformations of the data. That is, the optimal sampling scheme $\boldsymbol{\mu}^*$ and the statistical properties of the resulting estimator $\hat{\boldsymbol{\theta}}_{\!\boldsymbol{\mu}}$ should not depend on the choice of parameterisation, nor on the scaling or coding of the data prior to modelling. 
%Invariance properties of optimality criteria and corresponding optimal sampling schemes are discussed below and further in Section \ref{sec:another_look_at_invariance}.



It is widely known that the D-optimality criterion is invariant to the parameterisation of the model and to non-singular affine transformations of the data in the above sense. 
%Indeed, this follows immediately from \eqref{eq:cov_eta}–\eqref{eq:cov_zeta} since the determinant of a matrix product is the product of the determinants, and the factor depending on the design ($\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)$) is unaffected by the transformation.
In contrast, the A- and E-optimality criteria are sensitive to changes in the parameterisation or data, and hence lack such invariance properties (ref). An L-optimal design may or may not be parameterisation- and transformation-invariant, depending on whether or not the matrix $\mathbf{L}$ is adopted to the parameterisation of the problem and scaling of the data.
%in the sense of Proposition \ref{prop:invariance}. 



A typical situation where transformation- and parameterisation-invariant L-optimality criteria are encountered is when the optimality criterion is defined to capture a comparison or evaluation of specific scientific interest. As an example, consider the problem of estimating the mean difference between two subgroups in the data. An optimal design may in this context be defined using the c-optimality criterion. The group means $\bar y_0, \bar y_1$ may for instance be parameterised as $\bar y_i = \alpha_i = \beta_0 + \delta_i = \gamma_0 + \gamma_1 \times i$, where $i = 0$ or $1$. Clearly, the contrast vector for the c-optimality criterion depends on the choice of parameterisation. 
%The precise relation between the parameterisation and optimality criterion is formalised in Proposition \ref{prop:invariance}. 
Other examples of transformation- and parameterisation-invariant L-optimality criteria are discussed in Section \ref{sec:another_look_at_invariance}.



\subsection{Proof of Proposition \ref{prop:invariance}}

\paragraph{Proof of \ref{prop:parameterisation_invariance}}

Consider a one-to-one differentiable mapping $\boldsymbol{g}: \boldsymbol{\theta} \mapsto \boldsymbol{\eta}$. Let $\boldsymbol{\mu}^*_1$ be the minimiser of the function $\tr(\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)\mathbf{L}_1\mathbf{L}_1^T)$, and $\boldsymbol{\mu}^*_2$ the minimiser of the function $\tr(\boldsymbol{\Gamma}_{\!\boldsymbol{g}}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)\mathbf{L}\mathbf{L}^T) = \tr(\boldsymbol{J}_{\!\boldsymbol{g}}(\boldsymbol{\theta}_0)\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)\boldsymbol{J}_{\!\boldsymbol{g}}(\boldsymbol{\theta}_0)\T\mathbf{L}_2\mathbf{L}_2^T) = \tr(\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)\boldsymbol{J}_{\!\boldsymbol{g}}(\boldsymbol{\theta}_0)\T\mathbf{L}_2\mathbf{L}_2^T\boldsymbol{J}_{\!\boldsymbol{g}}(\boldsymbol{\theta}_0))$. These two objective functions are identical if and only if $\mathbf{L}_1 = \boldsymbol{J}_{\!\boldsymbol{g}}(\boldsymbol{\theta}_0)\T\mathbf{L}_2 \Leftrightarrow \boldsymbol{J}^{-1}_{\!\boldsymbol{g}}(\boldsymbol{\theta}_0)\T\mathbf{L}_2$. 

According to the result of Proposition \ref{prop:optimality_conditions}, and optimal sampling scheme for $\hat{\boldsymbol{\theta}}_{\!\boldsymbol{\mu}}$ is on the form \eqref{eq:mui} or \eqref{eq:powor_a}--\eqref{eq:powor_c}, with  
\[
c_i = ||\mathbf{L}\mathbf{H}(\boldsymbol{\theta_0})^{-1}\boldsymbol{\psi}(\boldsymbol{\theta}_0)||.
\]


% Note that the minimiser of the $\boldsymbol{\eta}_0$ of induced empirical risk $\ell_{0, \boldsymbol{g}}^*(\boldsymbol{\eta}) := \ell_0(g^{-1}(\boldsymbol{\eta}))$ is given by $\boldsymbol{\eta}_0=\boldsymbol{g}(\boldsymbol{\theta}_0)$ (ref). Similarly, the Hansen-Hurwitz empirical risk minimiser for induced empirical risk is given by $\hat{\boldsymbol{\eta}}_{\!\boldsymbol{\mu}} = \boldsymbol{g}(\hat{\boldsymbol{\theta}}_{\!\boldsymbol{\mu}})$  By the delta method (ref), the approximate covariance matrix for $\hat{\boldsymbol{\eta}}_{\!\boldsymbol{\mu}}$ is given by
% $\boldsymbol{J}_{\!\boldsymbol{g}}(\boldsymbol{\theta}_0)\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0))\boldsymbol{J}\T_{\!\boldsymbol{g}}(\boldsymbol{\theta}_0)$.
% Consider an L-optimality criterion with respect to $\boldsymbol{\theta}_0$ and $\mathbf{L} = \mathbf{L}_1$, and an L-optimality criterion with respect to $\boldsymbol{\eta}_0$ and $\mathbf{L} = \mathbf{L}_2$. The two resulting sampling schemes are coincide if and only if the corresponding coefficient $c_i$ in \eqref{eq:ci} for all $i \in \mathcal D$. Now, the L-optimality criterion with respect to $\boldsymbol{\theta}_0$ results in 
% \[
% c_i = 
% \bigr\rvert\bigr\rvert
% \mathbf{L}_1\T
% \mathbf{H}(\boldsymbol{\theta})^{-1}
% \boldsymbol{\psi}_i(\boldsymbol{\theta})\bigr\rvert\bigr\rvert^2_{2, \boldsymbol{\theta} = \boldsymbol{\theta}_0},
% \]
% and the optimality criterion with respect to $\boldsymbol{\eta}_0$ in
% \[
% c_i = 
% \bigr\rvert\bigr\rvert
% \mathbf{L}_2\T
% \boldsymbol{J}_{\!\boldsymbol{g}}(\boldsymbol{\theta}_0)
% \mathbf{H}(\boldsymbol{\theta})^{-1}
% \boldsymbol{\psi}_i(\boldsymbol{\theta})\bigr\rvert\bigr\rvert^2_{2, \boldsymbol{\theta} = \boldsymbol{\theta}_0}.
% \]
% These two expressions coincide if and only if $\mathbf{L}_1 = \boldsymbol{J}\T_{\!\boldsymbol{g}}(\boldsymbol{\theta}_0)
% \mathbf{L}_2 \Leftrightarrow \mathbf{L}_2 = \boldsymbol{J}^{-T}_{\!\boldsymbol{g}}(\boldsymbol{\theta}_0)
% \mathbf{L}_1$.


%The need for subsampling inevitably arises in a wide range of situations, including survey sampling, experiments with measurement-constraints, and analysis of massive datasets. We have presented a theory for optimal subsampling in a context that encompasses a broad range of estimation problems in statistics, including finite population inference, parametric density estimation, and regression modelling. Algorithms for finding optimal sampling schemes have been derived for a general class of optimality criteria, including A-, D-, L-, and $\Phi_r$-optimality. We have also presented a novel class of transformation- and parameterisation-invariant linear optimality criteria. These were derived through an expected-distance-minimising perspective on optimal design, using three natural and common choices of statistical distance functions: the empirical risk distance, Mahalanobis distance, and Kullback-Leibler divergence. Due to their computational tractability and good invariance properties, these optimality criteria may play an equally important role for data subsampling applications as D-optimality does in traditional experimental design. These invariant linear optimality criteria should be considered as standard, all-purpose options for optimal design in general subsampling applications.

% To summarise, we have presented a theory of optimal design for general data subsampling problems. The two major assumptions were that the target parameter is defined as the solution to an estimating equation, differentiable in a neighbourhood of that point, and the objective function is differentiable in a neighbourhood of the optimum. We have derived optimality criteria for a general class of optimality criteria under an assumption of differentiability near the optimum, and presented algorithms for finding optimal sampling schemes for multinomial sampling designs and Poisson sampling with and without replacement. We have studied optimal subsampling from distance minimising perspective, defined a corresponding class of expected-distance-minimising optimality criteria, and established equivalence to traditional optimality criteria. We have derived corresponding optimal sampling schemes for minimising the expected empirical risk distance, Kullback-Leibler divergence, and Mahalanobis distance from the obtained estimate the full data parameter. Moreover, these are shown in many cases to be equivalent or essentially identical. Importantly, this led us to derive a novel class of linear optimality criteria with good properties: computationally as efficient as A-optimality, practically as good as D-optimality with respect to invariance properties. Indeed, such L-optimal designs were proved by the invariant to non-singular affine transformations of the data and one-to-one differentiable transformations of the parameter. These invariant linear optimality criteria should be considered as a standard all-purpose option for optimal design in general subsampling applications.



% We focused in this paper on the choice of sampling scheme for a given family of sampling designs, including multinomial sampling designs and Poisson sampling with and without replacement. We note that multinomial sampling and Poisson sampling with replacement have identical asymptotic properties, whereas Poisson sampling has a slightly higher asymptotic efficiency. In practice, the choice of sampling design may be based on a joint consideration of the efficiency, computational, and practical advantages of different designs. In some applications, a conditional Poisson sampling design without replacement and fixed sample size may be desired. However, simple closed form expressions of the joint inclusion probabilities are not available in this case, rendering optimisation analytically and computationally unfeasible. Moreover, the sampling process is itself computationally demanding with this design, making this an intractable option when computational efficiency is crucial. The potential benefits of this design are expected to be negligible when the sampling fraction is small, as is the case in most practical situations where subsampling is invoked. If, however, a conditional Poisson sampling design is desired, an optimal Poisson sampling scheme may be used.  



% We also note that our presentation limited to unequal probability sampling with inverse probability weighting. The data subset selection problem has also been studied from the perspective of optimum experimental design in, e.g.,  \citet{Wynn1977, Wynn1982, Pronzato2006, Schein2007, Drovandi2017, Deldossi2022}. 



% Among the sampling designs considered, linear optimality criteria are preferred with respect to computational aspects. Indeed, in this case there is a closed form expression for the optimal sampling probabilities in with-replacement designs. For fixed size designs, a simple correction may be needed to ensure that a feasible solution with sampling probabilities less than or equal to one is obtained. On the other hand, most L-optimal sampling schemes suffer from lack of invariance to transformations of the data and re-parameterisation of the model. D-optimality, rendering the optimal sampling scheme unaffected by transformation- and parameterisation changes, is often preferred in this aspect. In our examples, our algorithm for finding a D-optimal sampling scheme converged to the optimal solution within xx–yy iterations. Hence, D-optimality is a feasible optimality criterion for data subsampling. 



% Our algorithm successfully found a locally E-optimal design in one our our examples. In this case, however, the optimality criterion was largely driven by a single parameter, and corresponded very closely to A- and c-optimality. In the two other examples, our methods failed to find an E-optimal design. On the other hand, the E-optimality criterion relies heavily on the parameterisation of the model and scaling of the data and hence inappropriate if an invariant design is desired. In fact, finding an E-optimal is hard also in the traditional experimental design context. 



% We have shown that D-optimality may be regarded as minimising an expected Mahalanobis distance form the estimate to target parameter. 



% A-optimality is simple and computationally tractable, but heavily influenced by the parameterisation of the model and scaling or coding of the data prior to modelling. 



% Our framework enables finding D-optimal designs for regression modelling, parametric density estimation, and finite population inference. 



% We have proven that under suitable conditions the D-optimality criterion is convex, and presented an efficient algorithm for finding D-optimal sampling schemes. In our examples the D-optimal design was found within x iterations. 



% We have presented a class of linear optimality criteria with equally good invariance properties as D-optimality at up to xx times lower computational demand. Indeed, analytical solutions exists and not iterative procedures needed. Hence, this is a suitable class of optimality criteria also in big data applications where the computation time needed to find an optimal design is a crucial issue. Moreover, this have been shown by examples to be closely related to Mahalanobis distance for multivariate analyses, and to leverage sampling for regression modelling. It is also equivalent to A-optimality after an appropriate change of variables.



%\section{Discussion}
%\label{sec:conclusion}

%The need for subsampling inevitably arises in a wide range of situations, including survey sampling, experiments with measurement-constraints, and analysis of massive datasets. We have presented a theory for optimal subsampling in a context that encompasses a broad range of estimation problems in statistics, including finite population inference, parametric density estimation, and regression modelling. Algorithms for finding optimal sampling schemes have been derived for a general class of optimality criteria, including A-, D-, L-, and $\Phi_r$-optimality. We have also presented a novel class of transformation- and parameterisation-invariant linear optimality criteria. These were derived through an expected-distance-minimising perspective on optimal design, using three natural and common choices of statistical distance functions: the empirical risk distance, Mahalanobis distance, and Kullback-Leibler divergence. Due to their computational tractability and good invariance properties, these optimality criteria may play an equally important role for data subsampling applications as D-optimality does in traditional experimental design. These invariant linear optimality criteria should be considered as standard, all-purpose options for optimal design in general subsampling applications.



%A general theory that describes the asymptotic properties of estimators from sequential subsampling designs in the full generality has to our knowledge not been presented and hence is requested. This topic, however, is 

%\newpage



%\pagebreak[4]


% To see this, consider an invertible differentiable transformation $\boldsymbol{g}: \boldsymbol{\theta}\mapsto \boldsymbol{g}(\boldsymbol{\theta}) = (g_1(\boldsymbol{\theta}), \ldots, g_d(\boldsymbol{\theta}))^T =: \boldsymbol{\eta}$ of the parameter $\boldsymbol{\theta}$. This transformation may be due to a re-parameterisation of the model, or induced by an affine transformation of the data, or a combination of both. In either case, the minimiser of the induced empirical risk $\ell_{0, \boldsymbol{g}}^*(\boldsymbol{\eta}) := \ell_0(\boldsymbol{g}^{-1}(\boldsymbol{\eta}))$ is given by $\boldsymbol{\eta}_0 = \boldsymbol{g}(\boldsymbol{\theta}_0)$ \citep[see, e.g.,][Theorem 7.2.10]{Casella2001}. Moreover, the corresponding estimator of $\boldsymbol{\theta}_0$ By the equivariance property of the ERM, the Hansen-Hurvitz ERM for $\boldsymbol{\eta}_0$ may be obtained as $\hat{\boldsymbol{\eta}}_{\!\boldsymbol{\mu}} = \boldsymbol{g}(\hat{\boldsymbol{\theta}}_{\boldsymbol{\mu}})$. By the delta method, the approximate covariance matrix of $\hat{\boldsymbol{\eta}}_{\!\boldsymbol{\mu}}$ is given by
% \begin{equation}
%     \label{eq:approximate_covariance_matrix_trans}
%     \boldsymbol{\Gamma}_{\!\boldsymbol{g}}(\boldsymbol{\mu}) = \boldsymbol{J}_{\!\boldsymbol{g}}(\boldsymbol{\theta})\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)\boldsymbol{J}_{\!\boldsymbol{g}}(\boldsymbol{\theta})^T\bigr\rvert_{\boldsymbol{\theta} = \boldsymbol{\theta}_0},
% \end{equation}
% where $\boldsymbol{J}_{\!\boldsymbol{g}}(\boldsymbol{\theta})$ is the Jacobian matrix of $\boldsymbol{g}(\boldsymbol{\theta})$, i.e. the $d \times d$ matrix with rows $\nabla_{\!\boldsymbol{\theta}}g_k(\boldsymbol{\theta})^T$ \citep[see, e.g.,][]{Sen1993}. We note that the expression \eqref{eq:approximate_covariance_matrix_trans} may also be obtained according to \eqref{eq:approximate_covariance} by direct differentiation of the induced empirical risk estimators $\hat{\ell}_{\boldsymbol{\mu}, \boldsymbol{g}}^* := \hat{\ell}_{\boldsymbol{\mu}}(\boldsymbol{g}^{-1}(\boldsymbol{\eta}))$ or $\hat{\ell}_{\boldsymbol{\mu}, \boldsymbol{h}}^{**} :=\sum_{i \in \mathcal S} \frac{S_i}{\mu_i}\ell(\boldsymbol{h}(\boldsymbol{x}_i, \boldsymbol{y}_i), \boldsymbol{\theta})$. We now define two important invariance properties of $\Phi$-optimal sampling schemes. 
%Note that $\boldsymbol{\Gamma}_{\boldsymbol{g}}(\boldsymbol{\mu})$ is positive definite whenever $\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)$ is, since the mapping $\boldsymbol{g}: \boldsymbol{\theta} \mapsto \boldsymbol{g}(\boldsymbol{\theta})$ is invertible and $\boldsymbol{J}_{\!\boldsymbol{g}}(\boldsymbol{\theta})$ full rank.  

%Let $\mathcal G$ denote the space of of one-to-one differentiable transformations on the parameter space $\boldsymbol{\Omega} \subset \mathbb{R}^d$, and $\mathcal H$ a space of affine invertible transformations acting on the data space $\mathcal X \times \mathcal Y \subset \mathbb{R}^{p} \times \mathbb{R}^r$. 



% We note first that the full-data empirical risk minimiser (ERM) $\boldsymbol{\theta}_0$ is equivariant to the parameterisation of the problem \eqref{eq:theta0}–\eqref{eq:ell0} in the following sense: for any one-to-one differentiable mapping $\boldsymbol{g}: \boldsymbol{\theta} \mapsto \boldsymbol{g}(\boldsymbol{\theta}) =: \boldsymbol{\eta}$, the minimiser of the induced empirical risk $\ell_{0, \boldsymbol{g}}^*(\boldsymbol{\eta}) := \ell_0(\boldsymbol{g}^{-1}(\boldsymbol{\eta}))$ is given by $\boldsymbol{\eta}_0 = \boldsymbol{g}(\boldsymbol{\theta}_0)$ \citep[see, e.g.,][Theorem 7.2.10]{Casella2001}. Similarly, every affine transformation $\boldsymbol{h}: (\boldsymbol{x}^T, \boldsymbol{y}^T) \mapsto (\boldsymbol{a} + \boldsymbol{x}^T\boldsymbol{B}, \boldsymbol{c} + \boldsymbol{y}^T \boldsymbol{D})$ induces a mapping $\boldsymbol{g}_{\boldsymbol{h}} \in \mathcal G$ on the parameter space, such that the minimiser of the induced empirical risk $\ell^{**}_{0, \boldsymbol{h}}(\boldsymbol{\theta}) := \sum_{i\in \mathcal D} \ell_i(\boldsymbol{h}(\boldsymbol{x}_i, \boldsymbol{y}_i),\boldsymbol{\theta})$ is given by $\boldsymbol{g}_{\boldsymbol{h}}(\boldsymbol{\theta}_0)$. If, for every $\boldsymbol{h}$ in some function space of affine transformations $\mathcal H$, the inference made from $\boldsymbol{\theta}_0$ and $\boldsymbol{g}_{\boldsymbol{h}}(\boldsymbol{\theta}_0)$ is qualitatively unchanged, i.e., does not depend on how the data was measured or coded prior to modelling, we say that $\boldsymbol{\theta}_0$ is equivariant to $\mathcal H$. A formal definition is provided below. 



% \begin{definition}[Equivariance of the empirical risk minimiser to affine transformations of the data] \hspace{1cm} \\
%     \label{def:affine_transformation_invariance}
%     Let $\boldsymbol{\theta}_0$ be defined according to \eqref{eq:theta0}–\eqref{eq:ell0}, and $\mathcal H$ a space of invertible affine transformations $\boldsymbol{h}: \{\boldsymbol{x}, \boldsymbol{y}\} \mapsto \{\boldsymbol{a} + \boldsymbol{B}\boldsymbol{x}, \boldsymbol{c} + \boldsymbol{D}\boldsymbol{y}\}$ on the data space $\mathcal X \times \mathcal Y$. We say that the empirical risk minimiser $\boldsymbol{\theta}_0$ is equivariant to $\mathcal H$ if for every $\boldsymbol{h} \in \mathcal H$ there exists a unique invertible differentiable mapping $\boldsymbol{g}_{\boldsymbol{h}} : \boldsymbol{\Omega} \to \boldsymbol{\Omega}$, not depending on the data $(\boldsymbol{x}_i, \boldsymbol{y}_i)_{i \in \mathcal D}$, such that the minimiser of the induced empirical risk $\ell_{0, \boldsymbol{h}}^{**}(\boldsymbol{\theta}) := \sum_{i\in \mathcal D} \ell_i(\boldsymbol{h}(\boldsymbol{x}_i, \boldsymbol{y}_i),\boldsymbol{\theta})$ is given by $\boldsymbol{g}_{\boldsymbol{h}}(\boldsymbol{\theta}_0)$.
% \end{definition}



% We need the equivariance property of Definition \ref{def:affine_transformation_invariance} since, in general, we cannot expect a $\Phi$-optimal sampling scheme $\boldsymbol{\mu}^*$ to be invariant to affine transformations of the data unless the ERM itself is equivariant to such transformations. We provide in Example \ref{example:regression_though_the_origin} a simple intuitive explanation to the meaning of equivariance according to this definition. 



% \begin{example}[Regression through the origin] \hspace{1cm} \\
% \label{example:regression_though_the_origin}
% Let $\hat{\beta}$ be the least squares estimate of the slope $\beta$ of the model $\hat y = \beta x$ given data $\{x_i, y_i\}_{i=1}^N$. Consider a linear transformation $h: y \mapsto k y$ with $k \ne 0$. The induced mapping, i.e., the slope of regression through the origin given data $\{x, ky_i\}_{i=1}^N$, can be obtained as $g_h(\hat{\beta}) = k\hat{\beta}$. Hence, the slope of regression through the origin is equivariant to non-singular linear transformations of the response variable. However, regression through the origin is not equivariant to arbitrary affine transformations $h: y \mapsto ky + m$ with $m \ne 0$. In this case the induced mapping, i.e., the slope of regression through the origin given data $\{x, ky_i + m\}_{i=1}^N$, can we written as $g_h(\hat\beta) = k\hat{\beta} + m (\sum_{i} x_i^2)^{-1}\sum_i x_i$. Hence, the induced mapping cannot be evaluated for $m \ne 0$ without additional knowledge about the data. Moreover, there exist for every $\hat{\beta}$ infinitely many $m$ such that $\mathrm{sign}(\hat{\beta}) \ne \mathrm{sign}(g_h(\hat{\beta}))$, i.e., that qualitatively alters the inference made. 
% \end{example}



% We also note that the choice of optimality criterion sometimes itself depends on the parameterisation of the model or coding of the data. We provide such an example below. 



% \begin{example}[Parameterisation-dependent c-optimality criterion] \hspace{1cm} \\
% \label{example:parameterisation_invariant_c_optimality}
% Consider a dataset $\{x_i, y_i\}_{i \in \mathcal D}$ with $\{x_i, y_i\} \in \{0, 1\} \times \mathbb{R}$. Assume that we are interested in the mean difference $\bar y_1 - \bar y_0$ between the two groups of elements $i  \in \mathcal D$ with $x_i = 1$ and $x_i=0$, where $\bar y_t = \sum_{i \in \mathcal D} y_i\mathbf{1}_{\{x_i = t\}}$, $t \in \{0, 1\}$. Let $\boldsymbol{\theta} = (\theta_1, \theta_2)^T$, $\boldsymbol{x}_i = (1-x_i, x_i)^T$, and $\boldsymbol{\theta}_0$ be the minimiser of the sum of squares $\ell_0(\boldsymbol{\theta}) := \sum_{i \in \mathcal D} (y_i - \boldsymbol{x}^T\boldsymbol{\theta})^2$. Similarly, let $\boldsymbol{\eta} = (\eta_1, \eta_2)^T$, $\boldsymbol{z}_i = (1, x_i)^T$, and $\boldsymbol{\eta}_0$ be the minimiser of the sum of squares $\ell_0^*(\boldsymbol{\eta}) := \sum_{i \in \mathcal D} (y_i - \boldsymbol{z}_i^T\boldsymbol{\eta})^2$. Assume that $\boldsymbol{\mu}^*$ is an optimal sampling scheme for estimating the mean difference $\bar y_1 - \bar y_0$. Then $\boldsymbol{\mu}^*$ is c-optimal for $\boldsymbol{\theta}_0$ with $\boldsymbol{c} = (-1, 1)^T$, and c-optimal for $\boldsymbol{\eta}_0$ with $\boldsymbol{c} = (0, 1)^T$. Indeed, if we let $\boldsymbol{c}(\boldsymbol{\theta}) = (-1, 1)^T$, $\boldsymbol{\mu}^*$ is c-optimal with respect to $ \boldsymbol{c}(\boldsymbol{A}\boldsymbol{\theta}) = \boldsymbol{A}^{-T}\boldsymbol{c}(\boldsymbol{\theta})$ for any non-singular linear transformation $\boldsymbol{A}\boldsymbol{\theta}$ of $\boldsymbol{\theta}$. 
% \end{example}



% Consider now an invertible differentiable transformation $\boldsymbol{g}: \boldsymbol{\theta}\mapsto \boldsymbol{g}(\boldsymbol{\theta}) = (g_1(\boldsymbol{\theta}), \ldots, g_d(\boldsymbol{\theta}))^T =: \boldsymbol{\eta}$ of the parameter $\boldsymbol{\theta}$. This transformation may be due to a re-parameterisation of the model, or induced by an affine transformation of the data, or both. Consider also an optimality criterion $\Phi$, which may depend on the parameterisation of the model and measurement-scale or coding of the data. We let $\Phi^*_{\!\boldsymbol{g}}$ and $\Phi^{**}_{\!\boldsymbol{h}}$ denote the corresponding optimality criteria under a re-parameterisation $\boldsymbol{g} : \boldsymbol{\theta}\mapsto \boldsymbol{g}(\boldsymbol{\theta})$ and affine transformation $\boldsymbol{h}: \{\boldsymbol{x}, \boldsymbol{y}\} \mapsto \{\boldsymbol{a} + \boldsymbol{B}\boldsymbol{x}, \boldsymbol{c} + \boldsymbol{D}\boldsymbol{y}\}$, respectively. By the equivariance property of the ERM, the Hansen-Hurvitz ERM for $\boldsymbol{\eta}_0$ may be obtained as $\hat{\boldsymbol{\eta}}_{\!\boldsymbol{\mu}} = \boldsymbol{g}(\hat{\boldsymbol{\theta}}_{\boldsymbol{\mu}})$. By the delta method, the approximate covariance matrix of $\hat{\boldsymbol{\eta}}_{\!\boldsymbol{\mu}}$ is given by
% \begin{equation}
%     \label{eq:approximate_covariance_matrix_trans}
%     \boldsymbol{\Gamma}_{\!\boldsymbol{g}}(\boldsymbol{\mu}) = \boldsymbol{J}_{\!\boldsymbol{g}}(\boldsymbol{\theta})\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)\boldsymbol{J}_{\!\boldsymbol{g}}(\boldsymbol{\theta})^T\bigr\rvert_{\boldsymbol{\theta} = \boldsymbol{\theta}_0},
% \end{equation}
% where $\boldsymbol{J}_{\!\boldsymbol{g}}(\boldsymbol{\theta})$ is the Jacobian matrix of $\boldsymbol{g}(\boldsymbol{\theta})$, i.e. the $d \times d$ matrix with rows $\nabla_{\!\boldsymbol{\theta}}g_k(\boldsymbol{\theta})^T$ \citep[see, e.g.,][]{Sen1993}. We note that the expression \eqref{eq:approximate_covariance_matrix_trans} may also be obtained according to \eqref{eq:approximate_covariance} by direct differentiation of the induced empirical risk estimators $\hat{\ell}_{\boldsymbol{\mu}, \boldsymbol{g}}^* := \hat{\ell}_{\boldsymbol{\mu}}(\boldsymbol{g}^{-1}(\boldsymbol{\eta}))$ or $\hat{\ell}_{\boldsymbol{\mu}, \boldsymbol{h}}^{**} :=\sum_{i \in \mathcal S} \frac{S_i}{\mu_i}\ell(\boldsymbol{h}(\boldsymbol{x}_i, \boldsymbol{y}_i), \boldsymbol{\theta})$. We now define two important invariance properties of $\Phi$-optimal sampling schemes. 
% %Note that $\boldsymbol{\Gamma}_{\boldsymbol{g}}(\boldsymbol{\mu})$ is positive definite whenever $\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)$ is, since the mapping $\boldsymbol{g}: \boldsymbol{\theta} \mapsto \boldsymbol{g}(\boldsymbol{\theta})$ is invertible and $\boldsymbol{J}_{\!\boldsymbol{g}}(\boldsymbol{\theta})$ full rank. 



% \begin{definition}[Invariance properties of $\Phi$-optimal sampling schemes] \hspace{1cm} \\
%     \label{def:invariance_properties}
%     Consider a function $\Phi: \mathbb{R}^{d\times d}\to \mathbb{R}$ and a family $\mathcal F$ of unequal probability sampling designs indexed by the sampling scheme $\boldsymbol{\mu}$. Let the expected size $\E[\sum_{i\in\mathcal D}S_i] = n$ be fixed, and denote by $\mathcal M_n$ the corresponding domain of $\boldsymbol{\mu}$. Let $\mathcal G$ denote the space of invertible differentiable transformations on the parameter space $\boldsymbol{\Omega}$,and $\mathcal H$ the largest class of invertible affine transformations on the data space $\mathcal X \times \mathcal Y$ such that the equivariance property of the ERM according to Definition \ref{def:affine_transformation_invariance} holds. For a transformation $\boldsymbol{h} \in \mathcal H$, denote by $\boldsymbol{g}_{\boldsymbol{h}} \in \mathcal G$ the induced mapping on the parameter space. For a function $\boldsymbol{g} \in \mathcal G$, let $\boldsymbol{\Gamma}_{\!\boldsymbol{g}}(\boldsymbol{\mu}) = \boldsymbol{J}_{\!\boldsymbol{g}}(\boldsymbol{\theta})\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)\boldsymbol{J}_{\!\boldsymbol{g}}(\boldsymbol{\theta})^T\bigr\rvert_{\boldsymbol{\theta} = \boldsymbol{\theta}_0}$ be the approximate covariance matrix the estimator $\boldsymbol{g}(\hat{\boldsymbol{\theta}}_{\!\boldsymbol{\mu}})$. We say that a $\Phi$-optimal sampling scheme $\boldsymbol{\mu}^* := \argmin_{\boldsymbol{\mu} \in \mathcal M_n} \Phi(\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0))$ is invariant to
%     \begin{enumerate}[label = \alph*)]
%         \item the parameterisation of the model if for every $\boldsymbol{g} \in \mathcal G$ it holds that
%         $
%         \boldsymbol{\mu}^* = \argmin_{\boldsymbol{\mu} \in \mathcal M_n} \Phi_{\!\boldsymbol{g}}^*(\boldsymbol{\Gamma}_{\boldsymbol{g}}(\boldsymbol{\mu})),
%         $
%         \label{list:parameterisation_invariance}
%         \item non-singular affine transformations of data if for every $\boldsymbol{h} \in \mathcal H$ it holds that 
%         $
%         \boldsymbol{\mu}^* = \argmin_{\boldsymbol{\mu} \in \mathcal M_n}  \Phi_{\boldsymbol{h}}^{**}(\boldsymbol{\Gamma}_{\boldsymbol{g}_{\boldsymbol{h}}}(\boldsymbol{\mu}))
%         $.
%         \label{list:data_transformation_invariance}
%         %, and
%         % \item equivariant to PO-WR and PO-WOR designs, if there exists some $k \ge 1$ such that $\boldsymbol{\mu}^*$ is $\Phi$-optimal for PO-WR $\Rightarrow \tilde{\boldsymbol{\mu}}^*$ is $\Phi$-optimal for PO-WOR, where $\tilde{\mu}_i^* = \min\{k\mu_i^*, 1\}$.
%     \end{enumerate}
% \end{definition}



% By the formulas for the approximate covariance matrix $\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)$ in Section \ref{sec:approximate_covariance_matrix}, the properties of PO-WR and MULT designs are asymptotically identical. Hence, and PO-WR optimal sampling scheme $\boldsymbol{\mu^*}$ is also optimal for the multinomial design, and vice versa. PO-WOR is different from two aspects, first because the sampling scheme is restricted to have $\mu_i \le 1$, and second because the approximate covariance matrix differ by a constant matrix $-\sum_{i \in \mathcal D} \nabla_{\!\boldsymbol{\theta}}\ell_i(\boldsymbol{\theta}_0)\nabla_{\!\boldsymbol{\theta}}\ell_i(\boldsymbol{\theta}_0)^T$. The last invariance property of Definition \ref{def:invariance_properties} states that the sampling scheme should be qualitatively unchanged to whether a with-replacement design (i.e., PO-WR or MULT) or without replacement design (i.e., PO-WOR) is used. In such circumstances, it suffices to perform the optimisation for PO-WR. The corresponding optimal sampling scheme for the PO-WOR design may then be obtained by a simple adjustment according to step \ref{step:mui}–\ref{step:output} in Algorithm \ref{alg:lopt}.  



% If the optimality criterion $\Phi$ is unaffected by the choice of parameterisation or coding of the data, the two invariance properties in Definition \ref{def:invariance_properties} are equivalent. Indeed, a sampling scheme that is invariant to re-parameterisation will in most cases also be invariant to affine transformations of the data, and vice versa. However, we provide in Section \ref{sec:application} an example of a linear optimality criterion that is invariant to the parameterisation of the model, but not to affine transformations of the data. 



%  (Proposition \ref{prop:invariance} \ref{list:D_invariance}). We have already seen in Example \ref{example:parameterisation_invariant_c_optimality} an example of a linear optimality criterion that is invariant to linear transformations of the parameter. More generally, L-optimal designs may or may not be parameterisation- and transformation-invariant, depending on whether or not the matrix $\mathbf{L}$ is adopted to the parameterisation of the problem in the sense of Proposition \ref{prop:invariance} \ref{list:L_invariance}. 



%In our last step towards a procedure for practically implementable optimal subsampling designs, we relax the requirements or prior information needed to for the anticipate variance minimising  in the previous section by  of a preliminary estimate of the target parameter $\boldsymbol{\theta}_0$ and auxliary model $f(\boldsymbol{x}, \boldsymbol{y}|\boldsymbol{z})$ we present a sequential optimal design procedure where the information needed to evaluate the anticipate variance is acquired gradually during the sampling process. 



%Also, \citet{Imberg2022a} considered optimal subsampling for case-control studies, and derived optimal sampling schemes solely based on previously available data and prior knowledge. In most cases, however, $\tilde{c}_i$ cannot be evaluated without observing any data. 



%The procedure outlined below is adopted from \citet{Imberg2022b}, which in turn has its inspiration in active machine learning. The idea in active learning is to obtain an optimal training dataset for machine learning and prediction by iterating between data collection and model updates. Some authors describes active learning as optimal experimental design for machine learning, although several alternative approaches to sample selection in active learning exists \cite[see, e.g.][for an excellent introduction]{Settles2012}. The typical situation in active learning is to collect data in a large number of small batches, often with only one new observation per sampling stage. This offers a great deal of flexibility on in the optimisation, but may in other contexts be either impractical or computationally overwhelming. In contrast, the standard approach in the big data literature is to adopt a two-stage sampling procedure with an initial simple random sample followed by a second, larger, unequal probability sample according to an optimal sampling scheme sampling \citep[see, e.g.][]{Ma2015, Wang2018}. Similar methods of sequential design also exists in the traditional optimal design literature (ref). 



% The method proceeds in $K$ iterations of sampling stages $k = 1, \ldots, K$, and selects in each iteration a batch of new instances from $\mathcal D$ according to a PO-WR, PO-WOR or multinomial sampling design of size $n_k$. To retain unbiasedness, all selected instances are retained in the sampling frame for all future iterations. At each step, we construct an unbiased estimator $\hat{\ell}_{\boldsymbol{\mu},k}(\boldsymbol{\theta}) = \sum_{i \in \mathcal L_k} \frac{S_{ki}}{\mu_{ki}}\ell_i(\boldsymbol{\theta})$ of the full-data empirical risk. These are then combined in a pooled estimate $\hat{\boldsymbol{\theta}}_{\!\boldsymbol{\mu}}^{(k)} = \argmin_{\boldsymbol{\theta} \in \boldsymbol{\Omega}} \hat{\ell}_{\boldsymbol{\mu}}^{(k)}(\boldsymbol{\theta})$, where $m_k := n_1 + \ldots + n_k$ is the total (expected) size after $k$ iterations. An estimator for $\boldsymbol{\theta}_0$ is then obtained as $\hat{\boldsymbol{\theta}}_{\!\boldsymbol{\mu}}^{(k)} = \argmin_{\boldsymbol{\theta} \in \boldsymbol{\Omega}} \hat{\ell}_{\boldsymbol{\mu}}^{(k)}(\boldsymbol{\theta})$. The method also include fitting an auxiliary model $f(\boldsymbol{x}, \boldsymbol{y}|\boldsymbol{z})$, which may be updated in each iteration to evaluate the anticipated variance at the current iteration.



% In the context of finite population inference, \citet{Imberg2022b} suggested three different methods for variance estimation:
% \begin{itemize}
%     \item Non-parametric importance weighted bootstrap.
%     \item Martingale method, which uses the square variation of the the estimates in each iteration.
%     \item Classical method, which uses classical survey sampling techniques to estimate the conditional covariance in each iteration, and constructs a combined estimate by pooling the estimates of all estimates so far. 
% \end{itemize}
% These procedures may also be applied for the more complex situation covered in this paper. A thorough treatment of this issue is, however, beyond the scope of this paper.



% \begin{algorithm}
%     \caption{Multi-stage $\Phi$-optimal sampling procedure}
%     \label{alg:multi_stage_sampling}
%     \textbf{Input}: Index set $\mathcal D$, optimality criterion $\Phi$, family of sampling designs (PO-WR, PO-WOR or multinomial), number of sampling stages $K$, batch sizes ${n_k}_{k=1}^K$. 
 
%     \textbf{Initialisation}: Let $m_0 = 0$, $\hat{\ell}_{\boldsymbol{\mu}}^{(0)}(\boldsymbol{\theta}) = \boldsymbol{0}$. 
     
%     \begin{algorithmic}[1]
%     \FOR{k = 1, 2, \ldots, K}

%         \STATE \textbf{Learning} (if $k > 1$):  Fit model $f(\boldsymbol{x}, \boldsymbol{y}|\boldsymbol{z})$ on the labelled dataset $\{(s_{ji}, \mu_{ji}, \boldsymbol{x}_i, \boldsymbol{y}_i, \boldsymbol{z}_i)\}_{i \in \mathcal L_j, j = 1, \ldots, k}$.  
%         \label{step:learning}
  	
%         \IF {k $> 1$ and \textbf{Learning} and \textbf{Estimation} steps were successful$^{\dagger}$} 

%             \STATE \textbf{Optimisation}: Calculate sampling scheme $\boldsymbol{\mu}_k$ to minimise the anticipated variance given current estimate $\hat{\boldsymbol{\theta}}_{\!\boldsymbol{\mu}}^{(k-1)}$ and model $f(\boldsymbol{x}, \boldsymbol{y}|\boldsymbol{z})$.

%         \ELSE
        
%             \STATE \textbf{Fallback}: Set $\mu_{ki} = n_k/N$ for all $i \in \mathcal D$.

%         \ENDIF
        
%         \STATE \textbf{Sampling}: Draw random sample $(s_{k1}, \ldots, s_{kN})$ according to input sampling design with sampling scheme $\boldsymbol{\mu}_k$
        
%         \STATE \textbf{Labeling}: Retrieve data $(\boldsymbol{x}_i, \boldsymbol{y}_i)$ for selected instance(s) $i \in \mathcal L_k := \{i \in \mathcal D: s_{ki} > 0\}$. 
		
%       	\STATE \textbf{Estimation}: Let 
%         \begin{gather*}
%             \hat{\ell}_{\boldsymbol{\mu},k}(\boldsymbol{\theta}) = \sum_{i \in \mathcal L_k} \frac{S_{ki}}{\mu_{ki}}\ell_i(\boldsymbol{\theta}), \quad
%             m_k = m_{k-1} + n_k, \\    
%             \hat{\ell}_{\boldsymbol{\mu}}^{(k)}(\boldsymbol{\theta}) = \frac{1}{m_k}\left(m_{k-1}\hat{\ell}_{\boldsymbol{\mu}}^{(k-1)}(\boldsymbol{\theta}) + n_k\hat{\ell}_{\boldsymbol{\mu},k}(\boldsymbol{\theta}) \right), \quad
%             \hat{\boldsymbol{\theta}}_{\!\boldsymbol{\mu}}^{(k)} = \argmin_{\boldsymbol{\theta} \in \boldsymbol{\Omega}} \hat{\ell}_{\boldsymbol{\mu}}^{(k)}(\boldsymbol{\theta})
%         \end{gather*}
%         \label{step:estimation}

%     \ENDFOR

%     \STATE \textbf{Output}: Final estimate $\hat{\boldsymbol{\theta}}_{\!\boldsymbol{\mu}}^{(k)}$, labelled dataset $\{(s_{ji}, \mu_{ji}, \boldsymbol{x}_i, \boldsymbol{y}_i, \boldsymbol{z}_i)\}_{i \in \mathcal L_j, j = 1, \ldots, k}$ of records with complete data. 
        
%     \end{algorithmic}

%     \medskip

%     \footnotesize{$^{\dagger}$By a successful estimation step we mean that an estimate $\hat{\boldsymbol{\theta}}_{\!\boldsymbol{\mu}}^{(k-1)}$ could be obtained in the previous iteration of the algorithm. By a successful learning step we mean that the model $f(\boldsymbol{x}, \boldsymbol{y}, \boldsymbol{z})$ could be fitted and reliable predictions obtained, as assessed by some measure of generalisation error (e.g., accuracy or coefficient of determination on hold-out data).}
% \end{algorithm}


\begin{itemize}
    \item Among Kiefer‘s $\xi_p$-criteria [see Kiefer (1974)] the E-optimality criterion is not differentiable if the multiplicity of the minimum eigenvalue of the information matrix of the
    optimal design is larger than 1. This property makes the determination of E-optimal designs to an extremely hard and challenging problem. In fact, an analytical construction of E-optimal designs for linear regression models is very difficult and has only been achieved in the one-dimensional case for a limited number of linear and nonlinear models [see Melas (1982), Dette (1993), Pukelsheim and Studden (1993), Dette and Haines (1994), among others].
    \item On the other hand, we can approach E-optimal designs using $\xi_p$-optimal designs as $|p| \rightarrow \infty$. We can show whenever $|p| \ge - \log d/ \log 0.95$, the $\xi_p$-optimal design has at least 95\% E-efficiency.
    \item volume of confidence ellipsoid propto prod root lambdas
    \item locally optimal designs. 
    \item Cochran (1973, pp. 771-772) described this dependency: "You tell me the value of 0, and I promise to design the best experiment for estimating 0"
\end{itemize}


For any choice of optimality criterion, the corresponding optimal sampling scheme can only be found and evaluated if $\mu_0, \sigma_0$ and $\{y_i\}_{i=1}^N$ are all known. The impact speed can in this case be modelled using the known input variables to the scenario generation, i.e., off-road glance duration and maximal deceleration during braking. The information needed to evaluate the above expectation may be acquired gradually using a two-stage, multi-stage or active sampling procedure, where all models and parameters involved are updated as more data becomes available. 



Similar to before, an truly optimal sampling scheme can only be found if the full-data parameter $\boldsymbol{\theta}_0$ and all responses $y_i$ are known.



As before, the information needed to evaluate the above expectation may be acquired gradually using a two-stage, multi-stage or active sampling procedure, where all models and parameters involved are updated as more data becomes available. See, e.g., \cite{Bach2007, Imberg2020} for an illustration in the active learning context. We note that this is guaranteed to produce strictly positive sampling probabilities, as long as $\sigma_e$ is bounded away from zero. 



Since the true gradients are unknown, we proceed as before by minimising a function of the anticipated variance. We illustrate this for L-optimality with $\mathbf{L} = \boldsymbol{H}(\boldsymbol{\theta}_0)\mathbf{V}(\boldsymbol{\theta}_0)^{-1/2}$. This amounts to replacing $c_i$ in \eqref{eq:ci_fps} by its expectation, treating the unknown value of $\boldsymbol{y}_i$ are a random variable $\boldsymbol{y}_i$. If we assume that $\boldsymbol{y}_i$ has mean $\hat{\boldsymbol{y}}_i$ and covariance matrix $\boldsymbol{\Sigma}_i$, we have by properties on quadratic forms \citep{Mathai1992} that
\[
\E[c_i] = w_i\left[(\hat{\boldsymbol{y}}_i - \boldsymbol{\theta}_0)^T\mathbf{V}(\boldsymbol{\theta}_0)^{-1} (\hat{\boldsymbol{y}}_i - \boldsymbol{\theta}_0) + \tr(\mathbf{V}(\boldsymbol{\theta}_0)^{-1}\boldsymbol{\Sigma}_i)\right].
\]
We note that this is strictly positive, and hence produces strictly positive sampling probabilities, as long as $\boldsymbol{\Sigma}_i$ is positive definite. In practice we replace $\boldsymbol{\theta}_0$ by a preliminary estimate $\tilde{\boldsymbol{\theta}}_0$. As before, the information needed to evaluate the above expectation may be acquired gradually using a two-stage or multi-stage or sampling procedure, where all models and parameters involved are updated as more data becomes available. \citet{Imberg2022b} developed an active sampling algorithm for optimal subsampling with respect to c-optimality in this particular context. 






%This is invariant both to the parameterisation of the problem, and to affine transformations of data data. Moreover, it is equivalent to A-optimality after a change of variables $\boldsymbol{y} \mapsto \mathbf{V}(\boldsymbol{\theta}_0)^{-1}\boldsymbol{y}$, i.e., after a principal component rotation or orthogonalisation of the data. Hence, the scaling of data and correlation between the variables of interest is automatically accounted for. For PO-WR and multinomial sampling, the corresponding optimal sampling schemes are on the form $\mu_i \propto \sqrt{c_i}$ with
% \begin{equation}
% \label{eq:ci_fps}
% c_i = w_i^2(\boldsymbol{y}_i - \boldsymbol{\theta}_0)^T\mathbf{V}(\boldsymbol{\theta}_0)^{-1}(\boldsymbol{y}_i - \boldsymbol{\theta}_0),
% \end{equation}
% i.e., with probabilities proportional to the Mahanalobis distance of $\boldsymbol{y}_i$ from the centre of the data, scaled by the observation weight $w_i$. 





%the parameterisation of the model and to non-singular affine transformation of the model matrix $\boldsymbol{X}$.



%In this case we may consider A-, D- and E-optimality, or c-optimality with $\mathbf{c} = (1, 0, 0)^T$ (optimised for mean impact speed reduction), $\mathbf{c} = (0, 1, 0)^T$ (optimised for mean injury risk reduction), or $\mathbf{c} = (0, 0, 1)^T$ (optimised for crash avoidance rate). A major disadvantage with A- and E-optimality is the strong dependence on the scaling of the data. Indeed, the impact speed reduction and injury risk reduction differs by orders of magnitude. Hence, both of these optimality criteria will be largely driven by the mean impact speed reduction, and one may expect A-, E- and c-optimality with $\mathbf{c} = (1, 0, 0)^T$ to be very similar.



%Consider also the L-optimality criterion with $\mathbf{L} = \mathbf{H}(\boldsymbol{\theta}_0)^{1/2}$, as suggested in \ref{sec:d_star_examples}. In this case the Hessian matrix is diagonal and this optimality criterion equivalent to A-optimality. Moreover, $\mathbf{H}(\boldsymbol{\theta}_0)$ is unaffected by non-singular affine transformations of the data. On the other hand, if we consider an re-parameterisation $\boldsymbol{g}: \boldsymbol{\theta} \mapsto \boldsymbol{g}(\boldsymbol{\theta})$, the Hessian with respect to the new parameterisation becomes 
%$\boldsymbol{J}_{\!\boldsymbol{g}}(\boldsymbol{\theta})\mathbf{H}(\boldsymbol{\theta})\boldsymbol{J}_{\!\boldsymbol{g}}(\boldsymbol{\theta})^T\bigr\rvert_{\boldsymbol{\theta} = \boldsymbol{\theta}_0}$. Hence, the L-optimality criterion with $\mathbf{L} = \mathbf{H}(\boldsymbol{\theta}_0)^{1/2}$ is invariant to the parameterisation of the problem, but not to affine transformations of the data. 


%Hence, we have that $\E[c_i] = h_{ii}(1-h_{ii})$, and the optimal sampling scheme is to sample with probability proportional to $\sqrt{h_{ii}(1-h_{ii})}$ evaluated at a preliminary estimate $\tilde{\boldsymbol{\theta}}_0$. 

%for when applied to homoscedastic models. The shrinkage factor $\sqrt{1-h_{ii}}$ is included to account for the fact that the residuals are smaller for high-leverage data points since these drive the fit towards the observed value of $y_i$. However, this factor is negligible when the number of parameters $d$ is small compared to the size $N$ of the initial dataset. 

%This is turn is the sa   model this change of variables corresponds to a principal component rotation, i.e, such that the $\boldsymbol{X} \mapsto \tilde{\boldsymbol{X}}$ where the columns of $\tilde{\boldsymbol{X}}$ are uncorrelated with unit variance.
%The latter, in a sense, accounts for deviations from the mean-variance relationship induced by the quasi-binomial model.Similar to D-optimality, both of these L-optimality criteria are invariant to non-singular linear transformations of the model matrix $\boldsymbol{X}$. 


% and 
% \begin{equation}
%     \label{eq:ci_response2}
%     c_i = (y_i - p_i(\boldsymbol{\theta}_0))^2 \boldsymbol{x}_i^T \mathbf{V}(\boldsymbol{\theta}_0)^{-1}\boldsymbol{x}_i,
% \end{equation}
% respectively. T
% he only difference between the two is the use of the model-based variances $p_i(\boldsymbol{\theta})(1-p_i(\boldsymbol{\theta}_0))$ in the former and squared deviations $(y_i - p_i(\boldsymbol{\theta}))^2$ in the latter. For a correctly specified model, these are virtually identical for large $N$. 


%or $\mathbf{L} = \mathbf{H}(\boldsymbol{\theta}_0)\mathbf{V}(\boldsymbol{\theta}_0)^{-1/2}$. 
%Among the traditional optimality criteria, D- and A-optimality arguably most appropriate in this context. However, A-optimality may be driven by a few influential parameters or subjects with a very steep response curve. In such cases it does not necessarily guarantee an overall good fit to the data. L-optimality could be used to optimise for estimating the response at a specific configuration of the input parameters. It is also possible to set up an L-optimality criterion to minimise, e.g., the mean squared error of the predictions over the entire response surface \citep[see, e.g.][]{Imberg2020}. Based on the findings in Section \ref{sec:d_star_optimality}, two candidates optimality criteria with good properties are L-optimality with $\mathbf{L} = \boldsymbol{X}^T\boldsymbol{W}(\boldsymbol{\theta}_0)^{1/2}$ or $\mathbf{L} = \mathbf{H}(\boldsymbol{\theta}_0)\mathbf{V}(\boldsymbol{\theta}_0)^{-1/2}$, where $\mathbf{V}(\boldsymbol{\theta}) = \sum_{i=1}^N \ell_i(\boldsymbol{\theta})\ell_i(\boldsymbol{\theta})^T = \boldsymbol{X}^T\widetilde{\boldsymbol{W}}(\boldsymbol{\theta}_0)\boldsymbol{X}$ and $\widetilde{\boldsymbol{W}}(\boldsymbol{\theta})$ the diagonal matrix with elements $(y_i - p_i(\boldsymbol{\theta}))^2$. 


%minimises the expected distance from $\boldsymbol{\theta}_0$ to $\hat{\boldsymbol{\theta}}_{\!\boldsymbol{\mu}}$ with respect to the empirical risk distance and Mahalanobis distance with dispersion matrix $\boldsymbol{\Sigma} = \mathbf{H}(\boldsymbol{\theta}_0)^{-1}$, whereas the second minimises the expected Mahalanobis distance with respect to $\boldsymbol{\Sigma} = \mathbf{H}(\boldsymbol{\theta}_0)^{-1}\mathbf{V}(\boldsymbol{\theta}_0)\mathbf{H}(\boldsymbol{\theta}_0)^{-1}$. 


%We note also that our sampling scheme is different from the usual probability proportional to size (pps) sampling scheme often used in survey sampling, which is this case would be $\mu_i\propto w_i |\hat y_i|$. The reason for this is twofold: first, we consider a non-linear rather than linear estimator for $\eta_0$. This produces the squared residual $(y_i - \eta_0)^2$ in \eqref{eq:mu_density_estimation}. Second, when considering the anticipated variance we must account for the we consider the anticipated variance, rather than the predicted . This resuls in the include of the residual variance $\sigma_e^2$. Hence, our method shrinks the sampling scheme towards a density sampling scheme with $\mu_i \propto w_i$ if the residual uncertainty is large, or to a uniform sampling scheme is all observation weights $w_i$ are equal. In contrast, traditional pps-sampling ignores the accuracy of the proxy $\hat y_i$ for $y_i$. 



%An obvious drawback with A- and E-optimality is the strong dependence on the parameterisation of the model. Some alternative parameterisations include the logarithmic mean and variance $(\mu, \sigma^2)$, or geometric mean and coefficient of variation $(e^{\mu}, \sqrt{e^{\sigma^2}}-1)$. All these produce equivalent models on the full-data, but may produce subsampling estimators with very different properties if A- or E-optimality is used. It is also not evident that the location parameter $\mu$ and scale parameter $\sigma$ are equally important when estimating the impact speed distribution, as implicitly assumed if A-optimality is used.


%The D-optimality criterion and L-optimality with $\mathbf{L} = \mathbf{H}(\boldsymbol{\theta}_0)^{1/2}$ and $\mathbf{L}= \mathbf{H}(\boldsymbol{\theta}_0)\mathbf{V}(\boldsymbol{\theta}_0)^{-1/2}$ are further invariant to the and to the parameterisation. 
%, whereas the natural parameterisation for $\boldsymbol{L}_z$ is the 
%of the model, if we assume that the columns of the $\mathbf{L}_z$-matrix are adopted to minimise the average variance of the estimated centiles of the fitted log-normal distribution under the specified parameterisation. 







%The above-mentioned target characteristics correspond to the three examples of inference problems presented in Section \ref{sec:introduction}. They will be studied from a subsampling perspective in Section \ref{sec:parametric_density_estimation}–\ref{sec:finite_population_inference} to illustrate and exemplify the presented methodology. 

    %The injury risk is related to the impact speed though a logistic function. 
    %The crash avoidance indicator is a binary variable taking the value 1 if there was a crash in the baseline scenario that was successfully avoided with the AEB system, and 0 otherwise.


                % \STATE Select a new random subsample of size $n_k$ according to the optimal sampling scheme derived in step 
            % \footnotesize\ref{step:optimal_sampling_scheme}.\normalsize
            % \STATE Update the auxiliary model.
            % \label{step:auxiliary_model}
                %Repeat steps \footnotesize\ref{step:optimal_sampling_scheme}–\ref{step:auxiliary_model} \normalsize
    %until the desired sample size or sufficient precision is reached.


    %In particular, a feasible global optimum for the D- and L-optimality criteria with respect to the anticipated covariance matrix always exist when $f(\boldsymbol{x}, \boldsymbol{y}|\boldsymbol{z})$ is non-degenerate, and may be found using Algorithm \ref{alg:lopt} and \ref{alg:linearisation} with the modifications described above.
%In the context above, this in turn correspond to overfitting in the learning step (ref). Hence, by avoiding overfitting we may avoid sampling selection probabilities too close to zero, obtain well-calibrated sampling schemes and avoid variance inflation due to incidentally large sampling weights. See also \citet{Imberg2022b} for further discussion on this topic. 


%Dependence of the coefficient matrix $\mathbf{L}$ on the the parameter $\boldsymbol{\theta}$ is in fact necessary to obtain transformation- and parameterisation invariance (Proposition \ref{prop:L_invariance}). 



        % on the data space $\mathcal X \times \mathcal Y$ induces a mapping $\boldsymbol{g}_{\boldsymbol{h}}$ on the parameter space $\boldsymbol{\Omega}$ such that 
        % %\begin{equation}                
        % %    \label{eq:transformation_invariance_assumption}
        % $
        % \frac{\partial^2\ell_{0, \boldsymbol{h}}(\boldsymbol{\theta})}{\partial\boldsymbol{\theta}\partial\boldsymbol{\theta}^T} = \boldsymbol{J}_{\!\boldsymbol{g}_{\boldsymbol{h}}}(\boldsymbol{\theta})^{-T}\mathbf{H}(\boldsymbol{\theta})\boldsymbol{J}_{\!\boldsymbol{g}_{\boldsymbol{h}}}(\boldsymbol{\theta})^{-1},
        % $
        %\end{equation}


        


%We will focus in this paper on the optimal choice of sampling scheme for a given class of sampling designs, e.g., PO-WR, PO-WOR and multinomial sampling. The choice of sampling design may then be based on a joint consideration of the efficiency and computational or practical advantages of different candidate designs. 



%Note that the asymptotic properties of the PO-WR and multinomial designs are identical, whereas the approximate covariance matrix for PO-WOR differ from PO-WR and MULT by a constant matrix $-\sum_{i \in \mathcal D} \nabla_{\!\boldsymbol{\theta}}\ell_i(\boldsymbol{\theta}_0)\nabla_{\!\boldsymbol{\theta}}\ell_i(\boldsymbol{\theta}_0)^T$.



%To simplify notation, we will write the approximate covariance matrix $\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)$ as $\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)$, emphasising the dependency of $\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)$ on the sampling scheme $\boldsymbol{\mu}$, but leaving the dependency on the full-data parameter $\boldsymbol{\theta}_0$ implicit. 
%Similarly, we write the gradients $\nabla_{\!\boldsymbol{\theta}}\ell_i(\boldsymbol{\theta})$ and $\nabla_{\!\boldsymbol{\theta}}\hat{\ell}_{\boldsymbol{\mu}}(\boldsymbol{\theta})$ as $\nabla_{\!\boldsymbol{\theta}}\ell_i$ and $\nabla_{\!\boldsymbol{\theta}}\hat{\ell}_{\boldsymbol{\mu}}$, respectively. 





% \begin{figure}[!htb]
%     \centering
%     \includegraphics[scale = 1]{Figures/nloptr.png}
%     \caption{Computation time needed to find an optimal PO-WR sampling scheme for estimating a scalar parameter $\theta_0$ using numerical optimisation. This example was implemented in \texttt{R} \citep{RCoreTeam2022} using the \texttt{nloptr} package \citep{nloptr}.}
%     \label{fig:nloptr}
% \end{figure}



         %\item The A-optimality criterion $\Phi(\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)) = \tr(\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0))$ is differentiable with respect to $\boldsymbol{\mu}$, and $\boldsymbol{\phi}(\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)) = \mathbf{I}_{d\times d}$.
        %\item The c-optimality criterion $\Phi(\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)) := \mathbf{c}^T\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)\mathbf{c}$ is differentiable with respect to $\boldsymbol{\mu}$, and $\boldsymbol{\phi}(\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)) = \mathbf{c}\mathbf{c}^T$.
       %\item Let $\Phi(\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)) = ||\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)||_F^2 = \tr(\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)^2)$ be the squared Frobenius norm of $\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)$. Then $\Phi$ is differentiable with respect to $\boldsymbol{\mu}$, and $\boldsymbol{\phi}(\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)) = 2\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)$.


           %\item Conditional Poisson sampling, CPO($\boldsymbol{\mu}$): $S_1, \ldots, S_N$ dependent with $S_i \sim \mathrm{Bernoulli}(\mu_i)$ with fixed sample size $n = \E[n] = \sum_{i\in \mathcal D} S_i = \sum_{i \in \mathcal D}\mu_i$, $\mu_i \in (0, 1]$. 


               % \begin{subequations}
    %     \begin{align}
    %         \label{eq:powor_a}
    %         \mu_i^* & = 1 \text{ for all $i \in \mathcal E$}, \\
    %         \label{eq:powor_b}
    %         \sqrt{c_i}/\mu_i^* & \ge \sqrt{c_j}/\mu_j^* \quad \text{for all $i \in \mathcal E$ and $j \in \mathcal D \setminus \mathcal E$},         \end{align}   
    % \end{subequations}
    % and
    % \setcounter{equation}{11}
    % \begin{subequations}
    %     \setcounter{equation}{2}
    %     \begin{align}
    %         \label{eq:powor_c}
    %         \mu^*_i & = (n - n_{\mathcal E}) \frac{\sqrt{c_i}}{\sum_{j \in \mathcal D \setminus \mathcal E} \sqrt{c_j}} \quad  \text{for all $i \in \mathcal D \setminus \mathcal E$}.
    %     \end{align}   
    % \end{subequations}


    


%Note that the matrix $\mathbf{L}^*$ in proposition \ref{prop:optimality_conditions} is not necessarily not unique, and may depend on both $\boldsymbol{\mu}^*$ and $\boldsymbol{\theta}_0$. As an example, consider the D-optimality criterion for which $\mathbf{L}_*$ may be taken as either the matrix square root or Cholesky factorisation of $\boldsymbol{\Gamma}(\boldsymbol{\mu}^*)$ (see Lemma \ref{lemma:differentiability} d)). But $\boldsymbol{\Gamma}(\boldsymbol{\mu}^*)$ depends on both $\boldsymbol{\mu}^*$ and $\boldsymbol{\theta}_0$, and so does in this case also $\mathbf{L}_*$. In contrast, for the A-optimality criterion we have that $\mathbf{L}_* = \mathbf{I}_{d \times d}$, which does not depend on $\boldsymbol{\theta}_0$ or $\boldsymbol{\mu}^*$. 



%We point out that \eqref{eq:ci} may result in $c_i= 0$. In such case, a feasible solution to the optimisation problem does not exist. Indeed, the optimal choice would then be to set $\mu_i = 0$, but this is an unfeasible solution since we require $\mu_i>0$ for unbiased inference. In practice, procedures that allow $c_i$ and $\mu_i$ to be zero or arbitrarily close to zero tend to produce estimators with unstable performance and should not be used. We will return to this issue in Section \ref{sec:practical_implementation}.


%The optimal value of $\mu_i$ would then be to set $\mu_i = 0$, which  of sampling scheme would then be to set $\mu_i$. The optimal solution would be to set the corresponding $\mu_i = 0$, which is an unfeasible solution.  This happens, e.g., if the gradient $\nabla_{\!\boldsymbol{\theta}}\ell_i(\boldsymbol{\theta})\rvert_{\boldsymbol{\theta} = \boldsymbol{\theta}_0}  = \boldsymbol{0}$, or when it is orthogonal to the row space of $\mathbf{L}_*\mathbf{H}^{-1}$. This in turn implies that partial derivative of $\Phi(\boldsymbol{\Gamma}(\boldsymbol{\mu}; \boldsymbol{\theta}_0))$ with respect to $\mu_i$ is zero for all $\mu_i \in \mathcal R$. Loosely speaking, this means that the gradient $\nabla_{\!\boldsymbol{\theta}}\ell_i(\boldsymbol{\theta})$ is aligned with $\mathbf{L}(\boldsymbol{u})$ and $\boldsymbol{\theta}_0$ is such a way that the element $i \in \mathcal D$ does not contribute to estimation. The optimal choice would be to set $\mu_i = 0$. However, this produces unfeasible solution. 



%Finding an optimal design and establishing global optimality for non-convex optimality criteria is very challenging. E-optimality is an example of such a non-convex optimality criterion. The $\Phi_p$-optimality criterion offers an opportunity to exploit convexity while emulating E-optimality, however. In particular, note that the $\Phi_1$-optimality criterion corresponds to A-optimality, which is convex by Proposition \ref{prop:convex}. On the other hand, the E-optimality criterion, obtained as the limit of the $\Phi_p$-optimality criterion as $p \rightarrow \infty$, is non-convex. Hence, we conjecture that there exists a critical value $p_0 \ge 1$, depending on the model and data, such that the $\Phi_p$-optimality criterion is convex for $p < p_0$, and non-convex for $p > p_0$. This may be used to iteratively approach E-optimality by solving a  sequence of convex optimisation problems for $\Phi_p$-optimality with increasing values of $p$ (Algorithm \ref{alg:Phi_p}).  



% \begin{algorithm}[!htb]
%     \caption{Sequential generation of $\Phi_p$-optimal sampling schemes}
%     \begin{algorithmic}[1] 
%     \label{alg:Phi_p}
%     \STATE Find $\Phi_1$-optimal (A-optimal) sampling scheme $\boldsymbol{\mu}^*_{1}$ according to Algorithm \ref{alg:lopt} with $\mathbf{L} = \mathbf{I}_{d \times d}$.
% 	\FOR{p = 2, 3, \ldots} 
% 	    \STATE Find $\Phi_p$-optimal sampling scheme $\boldsymbol{\mu}^*_{p}$ according to Algorithm \ref{alg:linearisation}, with $\boldsymbol{\mu}^*_{p-1}$ as initial value.
% 	    \IF{Algorithm \ref{alg:linearisation} did not converge}
% 	        \STATE \textbf{Stop}. \textbf{Return} $\boldsymbol{\mu}^*_{p-1}$.
% 	    \ENDIF
%     \ENDFOR
%     \end{algorithmic}
% \end{algorithm}

%We consider in this section the invariance (or lack of invariance) of $\Phi$-optimal sampling schemes to the parameterisation of the model and affine transformations of the data. 


%We say that an optimality criterion and corresponding optimal sampling scheme is invariant to the parameterisation of the model if it is invariant to transformations $\boldsymbol{\theta} \mapsto \boldsymbol{g}(\boldsymbol{\theta})$ for any one-to-one differentiable mapping $\boldsymbol{g}$ on the parameter space. Similarly, we say that it is invariant to non-singular affine transformations of the data if it is invariant to coordinate-wise affine transformations $(\boldsymbol{x}_i, \boldsymbol{y}_i) \mapsto (\boldsymbol{a} + \boldsymbol{B} \boldsymbol{x}_i,  \mathbf{c} + \boldsymbol{D} \boldsymbol{y}_i)$, where $\boldsymbol{B}$ and $\boldsymbol{D}$ are full rank.



    % \begin{enumerate}[label = \textit{\alph*)}]
    %     \item A D-optimal sampling scheme $\boldsymbol{\mu}^*$ is invariant to the parameterisation of the model and to non-singular affine transformations of the data.
    %     \label{list:D_invariance}
    %     \item 
    %     % \begin{enumerate}
    %     %     \item[(*)] 
    %     % \end{enumerate}
    %     %\item An L-optimal design is invariant to non-singular affine transformations of the data if and only if $\mathbf{L} = \mathbf{L}_{\boldsymbol{h}}(\boldsymbol{\theta})$ is a function of the affine transformation $\boldsymbol{h}$ such that for every $\boldsymbol{h} \in \mathcal H$ it holds that $\mathbf{L}_{\boldsymbol{h}}(\boldsymbol{\theta}) = \boldsymbol{J}_{\!\boldsymbol{g}_{\boldsymbol{h}}}(\boldsymbol{\theta})^{-T}\mathbf{L}(\boldsymbol{\theta})$.
    %     \label{list:L_invariance}
    % \end{enumerate}


          %\item For every $d^*$-optimality criterion, there exists a $\Phi$-optimality criterion $\Phi : \mathbb{R}^d \to \mathbb{R}$ such that $\boldsymbol{\mu}^*$ is $d^*$-optimal if and only if $\boldsymbol{\mu}^*$ is $\Phi$-optimal.
        %\item For every $\Phi$-optimality criterion, differentiable in a neighbourhood of the $\Phi$-optimal sampling scheme $\boldsymbol{\mu}^*$, there exists a function $d:\boldsymbol{\Omega}\to \mathbb{R}_+$ such that $\boldsymbol{\mu}^*$ is $\Phi$-optimal if and only if $\boldsymbol{\mu}^*$ is $d^*$-optimal with respect to $d$. 


           % \end{enumerate}
    % To motivate the remaining three choices of $\boldsymbol{\Sigma}$, we adopt a super-population viewpoint where may we think of $\boldsymbol{\theta}_0$ as an estimator of some super-population parameter $\boldsymbol{\theta}^*$. For a correctly specified parameter model this is the true parameter from which the full-data $(\boldsymbol{x}_i, \boldsymbol{y}_i)_{i=1}^N$ had been generated. For a semi-parametric, distribution-free or misspecified model, we may instead think of $\boldsymbol{\theta}^*$ as the limiting value of $\boldsymbol{\theta}_0$ as if additional data could be collected indefinitely. 
    % \begin{enumerate}

       % \item \textbf{Fisher-Rao geodesic distance}: Consider the space $\{f_{\boldsymbol{\theta}}: \boldsymbol{\theta} \in \boldsymbol{\Omega}\}$ of density functions $f_{\boldsymbol{\theta}}$, equipped with the Fisher information metric $\widetilde{\mathbf{H}}(\boldsymbol{\theta})$. On this manifold, the Fisher-Rao geodesic distance of $\boldsymbol{\theta}$ from $\boldsymbol{\theta}_0$ is defined as the length of the shortest path $\gamma$ from $\boldsymbol{\theta}_0$ to $\boldsymbol{\theta}$ with respect to $\mathbf{H}(\boldsymbol{\theta})$, i.e., $d_{\mathrm{FR}}(\boldsymbol{\theta}) := \min_{\gamma} \int_0^1 |\gamma'(t)|_{H} dt$, where $\gamma(0) = \boldsymbol{\theta}_0, \gamma(1) = \boldsymbol{\theta}$, and $|\boldsymbol{u}|_{H} := || \widetilde{\mathbf{H}}(\boldsymbol{\theta})^{1/2}\boldsymbol{u}||_2$. This is the natural geometry of the model space, in the sense that the Fisher-Rao geodesic distance is the only Riemannian metric (up to a multiplicative factor) that is invariant to the parameterisation of the model (ref Amari, Methods of Information Theory, Chapter 2.4). While this metric often is non-trivial to evaluate, we note that it may be approximated by the Mahalanobis distance with respect to the dispersion matrix $\boldsymbol{\Sigma} = \widetilde{\mathbf{H}}(\boldsymbol{\theta}_0)^{-1}$, i.e, $d_{\mathrm{FR}}(\boldsymbol{\theta}) = d_{\boldsymbol{\Sigma}}(\boldsymbol{\theta}) + o(\boldsymbol{\theta}-\boldsymbol{\theta_0})$ for parameter values $\boldsymbol{\theta}$ close to $\boldsymbol{\theta}_0$.
    % \label{list:fisher_rao}


       %This holds since $N^{-1}\mathbf{V}(\boldsymbol{\theta}) = \E_{y\sim f_{\boldsymbol{\theta}_0}(y|\boldsymbol{x})}[N^{-1}\mathbf{V}(\boldsymbol{\theta})] + O(N^{-1}) = N^{-1}\mathbf{H}(\boldsymbol{\theta}) + O(N^{-1})$, where the first equality follows from the law of large numbers and the second by properties of the Fisher information \citep[see, e.g.][]{Casella2001, Pawitan2001}.
    %\item The above-mentioned optimality criteria allow for a simplification of the coefficient $c_i$ in Proposition \ref{prop:optimality_conditions} as on the following form $c_i = \nabla_{\!\boldsymbol{\theta}}\ell_i(\boldsymbol{\theta})\mathbf{A}(\boldsymbol{\mu}^*; \boldsymbol{\theta})\nabla_{\!\boldsymbol{\theta}}\ell_i(\boldsymbol{\theta})\bigr\rvert_{\boldsymbol{\theta} = \boldsymbol{\theta}_0}$ with $\mathbf{A}(\boldsymbol{\mu}^*; \boldsymbol{\theta}) = \boldsymbol{\Gamma}(\boldsymbol{\mu}^*; \boldsymbol{\theta}_0)$ (D-optimality), $\mathbf{A}(\boldsymbol{\mu}^*; \boldsymbol{\theta}) = \mathbf{H}(\boldsymbol{\theta}_0)$ (L-optimality with $\mathbf{L} = \mathbf{H}(\boldsymbol{\theta}_0)^{1/2}$), $\mathbf{A}(\boldsymbol{\mu}^*; \boldsymbol{\theta}) = \mathbf{V}(\boldsymbol{\theta}_0)$ (L-optimality with $\mathbf{L} = \mathbf{H}(\boldsymbol{\theta}_0)\mathbf{V}(\boldsymbol{\theta}_0)^{1/2}$).


    

%To further emphasise the importance of these findings, consider a regular parametric model $f_{\boldsymbol{\theta}}(\boldsymbol{y}|\boldsymbol{x})$. Assume that $f_{\boldsymbol{\theta}}(\boldsymbol{y}|\boldsymbol{x})$ is correctly specified, i.e., that the data $(\boldsymbol{x}_i, \boldsymbol{y}_i)_{i=1}^N$ were generated according to the parametric family $f_{\boldsymbol{\theta}}(\boldsymbol{y}|\boldsymbol{x})$ for some $\boldsymbol{\theta} \in \boldsymbol{\Omega}$. While A-optimality minimises the expected Euclidean distance of $\hat{\boldsymbol{\theta}}_{\!\boldsymbol{\mu}}$ from $\boldsymbol{\theta}_0$, L-optimality with $\boldsymbol{L} = \widetilde{\mathbf{H}}(\boldsymbol{\theta}_0)^{1/2}$ minimises the expected distance with respect to the natural geometry of the model space, i.e., space of models $f_{\boldsymbol{\theta}}$ indexed by the parameter $\boldsymbol{\theta} \in \boldsymbol{\Omega}$ equipped with the Fisher information metric (ref). Furthermore, this is the only Riemannian metric on this space (up to a multiplicative constant) that is invariant to the parameterisation of the model. Indeed, the full-data Hessian matrix $\mathbf{H}(\boldsymbol{\theta}_0)$ and sums-of-squares-and-cross-products matrices $\mathbf{V}(\boldsymbol{\mu}; \boldsymbol{\theta}_0)$, $\mathbf{V}(\boldsymbol{\theta}_0)$ play a crucial role in obtaining parameterisation- and transformation-invariant sampling schemes. This will be further elucidated in the next section.  



%We show below that the sampling schemes obtained from the distance functions discussed in the previous are invariant to the parameterisation of the model and to affine transformations of the data. Moreover, they are generators of all such invariant designs in following sense:


    %Let the induced empirical risk $\ell^{**}_{0, \boldsymbol{h}}(\boldsymbol{\theta})$ of a non-singular affine transformation $\boldsymbol{h}$ of the data be defined as in Definition \ref{def:affine_transformation_invariance}. 


% Assume that $\boldsymbol{\mu}^*$ is $d^*$-optimal with respect to $d(\boldsymbol{\theta})$. Then $\boldsymbol{\mu}^*$ is also (locally) $\Phi$-optimal, where $\Phi$ is a solution to the differential equation $\frac{\partial \Phi(\boldsymbol{U})}{\partial \boldsymbol{U}}\bigr\rvert_{\boldsymbol{U} = \boldsymbol{\Gamma}(\boldsymbol{\mu}^*)} = \frac{\partial^2 d(\boldsymbol{\theta})}        {\partial\boldsymbol{\theta}\partial \boldsymbol{\theta}^T}\bigr\rvert_{\boldsymbol{\theta} = \boldsymbol{\theta}_0}$.
